Low-Step Multi-Commodity Flow Emulators

We introduce the concept of low-step multi-commodity flow emulators for any undirected, capacitated graph. At a high level, these emulators contain approximate multi-commodity flows whose paths contain a small number of edges, shattering the infamous flow decomposition barrier for multi-commodity flow. We prove the existence of low-step multi-commodity flow emulators and develop efficient algorithms to compute them. We then apply them to solve constant-approximate $k$-commodity flow in $O((m+k)^{1+\epsilon})$ time. To bypass the $O(mk)$ flow decomposition barrier, we represent our output multi-commodity flow implicitly; prior to our work, even the existence of implicit constant-approximate multi-commodity flows of size $o(mk)$ was unknown. Our results generalize to the minimum cost setting, where each edge has an associated cost and the multi-commodity flow must satisfy a cost budget. Our algorithms are also parallel.

==> arxivver/emulator-def.tex <==

\section{Step-Reducing Emulators: Definition}

The goal of this section is to show that, given any graph $G$, there exists another graph $G'$ such that any multi-commodity flow in $G$ can be routed in $G'$ with approximately the same congestion \emph{and} length, and moreover such flow in $G'$ can be routed via paths containing few edges. We call $G'$ a \emph{step-bounded congestion-length emulator} of $G$. Below, we introduce several terminologies to formalize this notion. 

\paragraph{Length Profiles of Flows.}

Let $L_{F}(u,v,\l)=\sum_{P\text{ is a }(u,v)\text{-path, }\l_{G}(P)\ge\l}F(P)$ denote the total value routed between $u$ and $v$ by $F$ via paths of length at least $\l$. Notice that $L_{F}(u,v,0)=D_{F}(u,v)$. We call $L_{F}$ the \emph{length-profile} of $F$. This notion allows us to compare the length of two flows.
\begin{defn}
[Comparing Length Profiles]Let $F$ and $F'$ be two multicommodity flows routing the same demand $D_{F}=D_{F'}$. We write $L_{F'}\preceq L_{F}$ and say that the length-profile of $F'$ is at most the length-profile of $F$ if $L_{F'}(u,v,\l)\le L_{F}(u,v,\l)$ for all $u,v,\l$. We write $L_{F'}\preceq s\cdot L_{F}$ and say that the length-profile of $F'$ is at most the length-profile of $F$ with slack $s$ if $L_{F'}(u,v,s\l)\le L_{F}(u,v,\l)$ for all $u,v,\l$.
\end{defn}

Let us verify that the notation above makes sense what we compare two flows $F$ and $F'$ when all flow paths of $F$ are long and flow paths of $F'$ are short. 
\begin{fact}
\label{fact:flow len all paths}Let $F$ and $F'$ be flows routing the same demand. If all flow paths of $F$ has length at least $h$ and all flow paths of $F'$ has length at most $h'$ (i.e. $\leng_{F'}\le h'$), then $L_{F'}\preceq(\frac{h'}{h})\cdot L_{F}$.
\end{fact}

\begin{proof}
Fix any $u$ and $v$. We will verify that $L_{F'}(u,v,(\frac{h'}{h})\cdot\l)\le L_{F}(u,v,\l)$ for all $\l$. For $\ell>h$, we have $L_{F'}(u,v,(\frac{h'}{h})\cdot\l)=0$ because $\leng_{F'}\le h'$. So the inequality is trivial. For $\l\le h$, we have $L_{F}(u,v,\l)=D_{F}(u,v)$. Since $L_{F'}(u,v,(\frac{h'}{h})\cdot\l)\le D_{F'}(u,v)=D_{F}(u,v)$ by definition, we have $L_{F'}(u,v,(\frac{h'}{h})\cdot\l)\le L_{F}(u,v,\l)$.
\end{proof}
To understand this definition more intuitively, suppose that both flow $F$ and $F'$ only assign unit value on paths of $G$ and $G'$ respectively (i.e. $F(P)\in\{0,1\}$ and $F'(P')\in\{0,1\}$ for all $P,P'$). $L_{F'}\preceq s\cdot L_{F}$ iff there is a bijection that maps each flow-path $P'$ in $G'$ to another flow-path $P$ in $G$ where $\ell_{G'}(P')\le s\cdot\ell_{G}(P)$. Notice that this ``path-wise'' comparison is more fine-grained than comparing the cost of the flow. Recall that the cost of flow $F$ is $\cost_{F}=\sum_{e}F(e)\ell(e)$. 
\begin{fact}
If $L_{F'}\preceq s\cdot L_{F}$, then $\cost_{F'}\le s\cdot\cost_{F}$. 
\end{fact}

\begin{proof}
\textbf{To prove. }

\textbf{Later Define Min-cost flow emulator. }

\textbf{Then show that Step-bounded Congestion-length emulator is a min-cost flow emulator. }

\textbf{Then, prove that min-cost flow emulator is composable.}
\end{proof}
%
Now, we are ready to formalize the notion of step-bounded congestion-length emulators. 
\begin{defn}
[Step-Reducing Emulators]\label{def:emu}Given a graph $G$ and a node-weighting $A$ in $G$, we say that $G'$ is a \emph{$t$-step congestion-length emulator} of $A$ with length slack $s$ and congestion slack $\kappa$ if there exist $s_{1},s_{2},\kappa_{1},\kappa_{2}\ge1$ where $s=s_{1}s_{2}$ and $\kappa=\kappa_{1}\kappa_{2}$ such that
\begin{enumerate}
\item Given a flow $F$ in $G$ routing a demand that respects $A$, there is a flow $F'$ in $G'$ routing the same demand where $\congest_{F'}\le\kappa_{1}\cdot\congest_{F}$, $L_{F'}\preceq s_{1}\cdot L_{F}$, and $\step_{F'}\le t$.
\item $G'$ can be embedded into $G$ with congestion $\kappa_{2}$ and length slack $s_{2}$.%
\begin{comment}
\begin{enumerate}
\item Given a flow $F'$ in $G'$, there is a flow $F$ in $G$ routing the same demand where $\congest_{F}\le\kappa_{2}\cdot\congest_{F'}$, $L_{F}\preceq s_{2}\cdot L_{F'}$. \textbf{(SAY THAT there is an embedding instead?) }
\end{enumerate}
\end{comment}
\end{enumerate}
\end{defn}

We write sometimes just say that $G'$ is a $t$-step emulator of $G$ for short. 

Below, we define a variant of step-bounded emulator. The first condition focuses only on flow of length at most $h$. The second condition remains the same as \ref{def:emu}.
\begin{defn}
[Step-Reducing $h$-Length Emulators]\label{def:h-len emu}Given a graph $G$, we say that $G'$ is an\emph{ $t$-step $h$-length emulator} of $G$ with length slack $s$ and congestion slack $\kappa$ if there exist $s_{1},s_{2},\kappa_{1},\kappa_{2}\ge1$ where $s=s_{1}s_{2}$ and $\kappa=\kappa_{1}\kappa_{2}$ such that
\begin{enumerate}
\item Given a flow $F$ in $G$ where $\leng_{F}\le h$, there is a flow $F'$ in $G'$ routing the same demand where $\congest_{F'}\le\kappa_{1}\cdot\congest_{F}$, $\leng_{F'}\le s_{1}\cdot h$, and $\step_{F'}\le t$.
\item $G'$ can be embedded into $G$ with congestion $\kappa_{2}$ and length slack $s_{2}$.%
\begin{comment}
Given a flow $F'$ in $G'$, there is a flow $F$ in $G$ routing the same demand where $\congest_{F}\le\kappa_{2}\cdot\congest_{F'}$, $L_{F}\preceq s_{2}\cdot L_{F'}$.
\end{comment}
\item Edges in $G'$ have the same length.
\end{enumerate}
We also say that $G'$ has length slack $(s_{1},s_{2})$ and congestion slack $(\kappa_{1},\kappa_{2})$. 
\end{defn}

The third condition requiring that edges in $G'$ have uniform length is crucial. This will allow us to bootstrap the construction for\emph{ }$t$-step $h$-length emulator for large $h$ to $t$-step $h'$-length emulator with small $h'\le n^{\eps}$. 


==> arxivver/emulator_exist.tex <==


\section{Step-Bounded Emulators: Existence}

\label{sec:emu}

The goal of this section is to show that, given any graph $G$, there exists another graph $G'$ such that any multi-commodity flow in $G$ can be routed in $G'$ with approximately the same congestion \emph{and} length, and moreover such flow in $G'$ can be routed via paths containing few edges. We call $G'$ a \emph{step-bounded congestion-length emulator} of $G$. 


We write sometimes just say that $G'$ is a $t$-step emulator of $G$ for short. The main theorem of this section is as follows.
\begin{thm}
\label{thm:emu}Given any graph $G$ and parameter $t$, there exists a $O(t^{2})$-step emulator $G'$ for $G$ with length slack $O(t^{4})$ and congestion slack $\poly(t)N^{O(1/t)}$. 

Moreover, suppose $\l_{G}(e),u_{G}(e)\in\mathbb{Z}_{>0}$ for all $e\in E(G)$. Then, for all $e\in E(G')$, $\l_{G'}(e)\in\mathbb{Z}_{>0}$, $u_{G'}(e)\in\frac{1}{h}\mathbb{Z}_{>0}$, $\sum_{e\in E(G')}u_{G'}(e)\le\sum_{e\in E(G)}u_{G}(e)N^{O(1/t)}$, and $\diam(G')\le O(t^{2})\cdot\diam(G)$.
\end{thm}

Below, we define a cruder variant of step-bounded emulator. The first condition focuses only on flow of length at most $h$. The second condition remains the same as \ref{def:emu}.
\begin{definition}
\label{def:h-len emu}Given a graph $G$, we say that $G'$ is an\emph{ $t$-step $h$-length emulator} of $G$ with length slack $s$ and congestion slack $\kappa$ if there exist $s_{1},s_{2},\kappa_{1},\kappa_{2}\ge1$ where $s=s_{1}s_{2}$ and $\kappa=\kappa_{1}\kappa_{2}$ such that \textcolor{blue}{Jason: $s$ and $\kappa$ are not used anywhere}
\begin{enumerate}
\item Given a flow $F$ in $G$ where $\leng_{F}\le h$, there is a flow $F'$ in $G'$ routing the same demand where $\congest_{F'}\le\kappa_{1}\cdot\congest_{F}$, $\leng_{F'}\le s_{1}\cdot h$, and $\step_{F'}\le t$.
\item Given a flow $F'$ in $G'$, there is a flow $F$ in $G$ routing the same demand where $\congest_{F}\le\kappa_{2}\cdot\congest_{F'}$, $L_{F}\preceq s_{2}\cdot L_{F'}$. \textcolor{blue}{Jason: $L_F$ is $\leng_F$?}
\end{enumerate}
We also say that $G'$ has length slack $(s_{1},s_{2})$ and congestion slack $(\kappa_{1},\kappa_{2})$.
\end{definition}

Our main technical contribution of this part is, in fact, showing the existence of step-bounded $h$-length emulator. 
\begin{thm}
\label{thm:h leng emu}Given any graph $G$ and parameters $h$ and $t$, there exists a $O(t^{2})$-step $h$-length emulator $G'$ for $G$ with length slack $O(t^{4})$ and congestion slack $\poly(t)N^{O(1/t)}$. 

Moreover, suppose $\l_{G}(e),u_{G}(e)\in\mathbb{Z}_{>0}$ for all $e\in E(G)$. Then, for all $e\in E(G')$, $\l_{G}(e)=h$, $u_{G}(e)\in\frac{1}{h}\mathbb{Z}_{>0}$ and $\sum_{e\in E(G')}u_{G'}(e)\le\sum_{e\in E(G)}u_{G}(e)N^{O(1/t)}$.
\end{thm}

We emphasize edges in $G'$ have a uniform length of $h$. This will be very useful later. We will show that \ref{thm:emu} follows easily from \ref{thm:h leng emu} later.


\subsection{Useful Facts }

Here, we state several facts that will be useful for constructing step-bounded emulator.

Below, we show that we can compare the length-profile between two flows if we can decompose and compare them. 
\begin{prop}
\label{prop:len decompose}Let $F=F_{1}+F_{2}$ and $F'=F'_{1}+F'_{2}$ be two flows in $G$ that can be decomposed such that $D_{F_{1}}=D_{F'_{1}}$ and $D_{F_{2}}=D_{F'_{2}}$. If $L_{F'_{1}}\preceq s_{1}\cdot L_{F_{1}}$ and $L_{F'_{2}}\preceq s_{2}\cdot L_{F_{2}}$, then $L_{F'}\preceq s\cdot L_{F}$ where $s=\max\{s_{1},s_{2}\}$.
\end{prop}

\begin{proof}
For any $u,v\in V$ and $\l$, we have $L_{F'}(u,v,s\l)=L_{F'_{1}}(u,v,s\l)+L_{F'_{2}}(u,v,s\l)\le L_{F'_{1}}(u,v,s_{1}\l)+L_{F'_{2}}(u,v,s_{2}\l)\le L_{F_{1}}(u,v,\l)+L_{F_{2}}(u,v,\l)=L_{F}(u,v,\l)$.
\end{proof}
We define the \emph{edge-demand} $D_{E(G)}$ of $G$ such that $D_{E(G)}(v,w)=u_{G}(v,w)$ for all $(v,w)\in E(G)$. A \emph{canonical flow} for routing $D_{E(G)}$ simply routes $D_{E(G)}(v,w)$ value of flow through the single edge $(v,w)$. Observe that the canonical flow of $D_{E(G)}$ has congestion exactly $2$.

Next, suppose we have two graphs $G$ and $G'$ and we want to show that any demand routable in $G'$ is also routable in $G$ with similar congestion and length (and we do not care about the step). It is enough to focus on routing the edge-demand of $G'$ in $G$ with small congestion and length.
\begin{prop}
\label{prop:edge demand}Let $\widehat{F}'$ be the canonical flow for routing the edge-demand $D_{E(G')}$ of $G'$. Suppose there exists a flow $\Fhat$ in $G$ that routes $D_{E(G')}$ where $\congest_{\Fhat}\le\kappa\cdot\congest_{\Fhat'}=2\kappa$ and $L_{\Fhat}\preceq s\cdot L_{\Fhat'}$. Then, for any flow $F'$ in $G'$, there exists a flow $F$ in $G$ that routes $D_{F'}$ where $\congest_{F}\le2\kappa\cdot\congest_{F'}$ and $L_{F}\preceq s\cdot L_{F'}$.
\end{prop}

\begin{proof}
Our strategy is as follows. For each pair $(v,w)$ and each $(v,w)$-flow-path $P'$ of $F'$, we will construct a $(v,w)$-flow $f_{P'}$ of value $\val(f_{P'})=F'(P')$ and length at most $s\cdot\l_{G'}(P')$. Let $F=\sum_{P':F'(P')>0}f_{P'}$. It is clear that $D_{F}=D_{F'}$ and $L_{F}\preceq s\cdot L_{F'}$. We will later bound $\congest_{F}$ but this will follow from the specifics of our construction.

Now, we describe the construction of $f_{P'}$. Consider each edge $(x,y)\in P'$. Let $\fhat_{(x,y)}$ be the $(x,y)$-flow of $\Fhat$ scaled down so that $\val(\fhat_{(x,y)})=F'(P')$. Then, $f_{P'}$ is the ``concatenation'' of $\fhat_{(x,y)}$ for all $(x,y)\in P'$. Therefore, $f_{P'}$ is a $(v,w)$-flow of value $F'(P')$. Now, we bound the length of $f_{P'}$. For each $(x,y)\in P'$, recall that the $(x,y)$-flow of $\Fhat'$ routes through the single edge $(x,y)$ of length of $\l_{G'}(x,y)$. As $L_{\Fhat}\preceq s\cdot L_{\Fhat'}$, the length of $(x,y)$-flow of $\Fhat$ is at most $s\cdot\l_{G'}(x,y)$. But $\fhat_{(x,y)}$ is simply the $(x,y)$-flow of $\Fhat$ after scaling. So the length of $\fhat_{(x,y)}$ is $s\cdot\l_{G'}(x,y)$ as desired.

It remains to analyze the congestion. Assume w.l.o.g. that the flow $F'$ in $G'$ has congestion $\congest_{F'}=1$. For each edge $(x,y)\in E(G')$, the construction above adds the $(x,y)$-flow of $\Fhat$ into $F$ with total value $\sum_{P':(x,y)\in P'}F'(P')=F'(x,y)\le u_{G'}(x,y)$ as $\congest_{F'}=1$. By definition of $\Fhat$ which is a flow that routes the edge-demand $D_{E(G')}$ of $G'$, even if we route the $(x,y)$-flow of $\Fhat$ of value exactly $u_{G'}(x,y)=D_{E(G')}(x,y)$ simultaneously for all $(x,y)\in E(G')$, the congestion would be at most $2\kappa$. So the congestion of $F$ is also at most $2\kappa$.
\end{proof}
The following lemma shows how to construct a $t$-step emulator given $t$-step $2^{i}$-length emulator for each $i$, where each emulator has the same slack $(s_{1},s_{2})$ and $(\kappa_{1},\kappa_{2})$.
\begin{lem}
\label{lem:reduc to h leng emu}For $i\in[0,\log N]$, let $G'_{i}$ be a $t$-step $2^{i}$-length emulator of $G$ with length slack $(s_{1},s_{2})$ and congestion slack $(\kappa_{1},\kappa_{2})$. Let $G'=\biguplus_{i}G'_{i}$. Then $G'$ is a $t$-step emulator of $G$ with length slack $(2s_{1},s_{2})$ and congestion $(\kappa_{1},\kappa_{2}2\log n)$.
\end{lem}

\begin{proof}
We will argue the following:
\begin{enumerate}
\item Given a flow $F$ in $G$ with congestion $1$, there is a flow $F'$ routing $D_{F}$ in $G'$ where $\congest_{F'}\le\kappa_{1}$, $L_{F'}\preceq2s_{1}\cdot L_{F}$, and $\step_{F'}\le t$.
\item Given a flow $F'$ in $G'$ with congestion $1$, there is a flow $F$ routing $D_{F'}$ in $G$ where $\congest_{F}\le\kappa_{2}\cdot2\log N$ and $L_{F}\preceq s_{2}\cdot L_{F'}$.
\end{enumerate}
For the first point, given $F$, we decompose $F=F_{0}+\dots+F_{\log N}$ so that $F_{0}$ contains all flow paths of length at most $1$ and $F_{i}$ contains all flow paths $P$ of $F$ where $2^{i-1}<\ell(P)\le2^{i}$ for $i\ge1$. For each flow $F_{i}$ in $G$, by \ref{def:h-len emu}, there is a flow $F'_{i}$ routing $D_{F_{i}}$ in $G'_{i}$ with $\congest_{F'_{i}}\le\kappa_{1}$, $\leng_{F'_{i}}\le s_{1}\cdot2^{i}$, and $\step_{F'_{i}}\le t$. By \ref{fact:flow len all paths}, we have that $L_{F'_{i}}\preceq2s_{1}\cdot L_{F_{i}}$. Let $F'=F'_{0}+\dots+F'_{\log N}$ be a flow in $G'$. We have $\congest_{G',F'}\le\max_{i}\congest_{G'_{i},F'_{i}}\le\kappa_{1}$ because $G'$ is a disjoint union of $G'_{i}$. Next, since $F=\sum_{i}F_{i}$ and $F'=\sum_{i}F'_{i}$ where $F_{i}$ and $F'_{i}$ routes the same demand, we have $L_{F'}\preceq2s_{1}\cdot L_{F}$ by \ref{prop:len decompose}. Lastly, we clearly have $\step_{F'}\le t$. This completes the proof of the first point.

For the second point, in the light of \ref{prop:edge demand}, we consider the edge-demand $D_{E(G')}$ of $G'$ and let $F'$ denote the canonical flow in $G'$ routing it. Recall that flow paths of $F'$ only route through a single edge of $G'$. We decompose $F'=F'_{0}+\dots+F'_{\log N}$ where $F'_{i}$ is a subflow of $F'_{e}$ routed through edges of $G'_{i}$. By \ref{def:h-len emu}, there exists $F_{i}$ routing $D_{F'_{i}}$ in $G$ where $\congest_{F_{i}}\le\kappa_{2}\cdot\congest_{F'_{i}}\le\kappa_{2}$ and $L_{F_{i}}\preceq s_{2}\cdot L_{F'_{i}}$. Now, let $F=F_{0}+\dots+F_{\log N}$ be a flow in $G$. Observe that $F$ routes $D_{F}=\sum_{i}D_{F_{i}}=\sum_{i}D_{F'_{i}}=D_{F'}$. Also, we have that $\congest_{G,F}\le\sum_{i}\kappa_{2}\congest_{G,F_{i}}\le\kappa_{2}\log N$ and $L_{F_{e}}\preceq s_{2}\cdot L_{F'_{e}}$ by \ref{prop:len decompose}. Thus, we have shown how to route the edge-demand of $G'$ in $G$ via $F$. By \ref{prop:edge demand}, this completes the second point.
\end{proof}
%
\begin{comment}
Each $G'_{i}$ might not have exactly the same slack tuple $(s_{1},s_{2})$ and $(\kappa_{1},\kappa_{2})$. This is can be handled easy by scaling.
\begin{cor}
\label{lem:emu reduc}For $i\in[0,\log N]$, let $G'_{i}$ be a $t$-step $2^{i}$-length emulator of $G$ with length slack $s$ and congestion slack $\kappa$. There is a $t$-step emulator $G'$ of $G$ with length slack $O(s)$ and congestion $O(\kappa\log N)$.
\end{cor}

\begin{proof}
By the lemma above, it suffices to scale up length and congestion of $G'_{i}$ so that all $G'_{i}$ have approximately the same slack bounds $(s_{1},s_{2})$ and $(\kappa_{1},\kappa_{2})$ where $s=\Theta(s_{1}s_{2})$ and $\kappa=\Theta(\kappa_{1}\kappa_{2})$. First, we round up length and congestion of every each in each $G'_{i}$ to a power of $2$. This will affect the slack up to a factor of $2$. Then, by scaling up the length and capacity of $G'_{i}$ by some powers of $2$ which is at most $2^{\log N}=N$, we are done.
\end{proof}
\end{comment}

\subsection{Construction and Analysis}
\begin{itemize}
\item \textbf{TODO: prove the sparsity of $G'$ too (using a star router). Extend to any node-weighting $A_{0}=A$ for general $A$.}
\end{itemize}
In this section, we show a construction of $t$-step $h$-length emulator. For any node weighting $A$, let $\router(A,t_{\rt},\kappa_{\rt})$ denote a $t_{\rt}$-step $\kappa_{\rt}$-congestion router for $A$ from \ref{lem:router expander}. We assign $t_{\rt}\gets t$ and $\kappa_{\rt}=O(t)$ in this section. 

\begin{algorithm}
Set $A_{0}\gets\deg_{G}$, $h_{\cov}\gets4h$, $h_{\diam}\gets8th$, $s_{\decomp}\gets t$, $\beta\gets h_{\diam}s_{\decomp}/h=8t^{2}$.
\begin{enumerate}
\item For $1\le i\le2t$: 
\begin{enumerate}
\item Let $C_{i}$ be a $\beta$-linked $(h_{\diam},s_{\decomp},\phi,\kappa_{\decomp})$-decomposition for $A_{i-1}$ from \ref{thm:expdecomp exist} where $\kappa_{\decomp}=N^{O(1/t)}\log N$ and $\phi=\frac{1}{2\beta\kappa_{\decomp}N^{1/t}}$.
\item Let $B_{i}=A_{i-1}+\beta\deg_{C_{i}}$ and $A_{i}=\beta\deg_{C_{i}}$.
\item Let $\N_{i}$ be a neighborhood cover of $G-C_{i}$ from \ref{thm:cover basic} with covering radius $h_{\cov}$, diameter $h_{\diam}$, and width $\omega=N^{O(1/t)}\log N$.
\item Let $E'_{i}=\bigcup_{S\in\cluster(\N_{i})}\router(B_{i,S},t_{\rt},\kappa_{\rt})$ where $B_{i,S}(v)=B_{i}(v)$ if $v\in S$, otherwise $B_{i,S}(v)=0$.
\end{enumerate}
\item Return $G'$ where $E(G')=\cup_{i}E'_{i}$ and $\ell_{G'}(e)=h$ for all $e\in E(G')$.
\end{enumerate}
\caption{\label{alg:emu}$\textsc{Emulator}(G,t,h)$}
\end{algorithm}

\textbf{}%
\begin{comment}
\textbf{Can we set $\beta$ very close to $1/\phi?$ No, because we want each level to shrink.}
\end{comment}

Let us start with basic technical observations on \ref{alg:emu}.
\begin{prop}
\label{prop:basics}We have the following:
\begin{enumerate}
\item For all $i$ and $v$, $A_{i}(v)$ and $B_{i}(v)$ are non-negative multiples of $\frac{1}{h}$.
\item Let $H_{i,S}=\router(B_{i,S},t_{\rt},\kappa_{\rt})$. We have $\deg_{H_{i,S}}\le\Delta\cdot B_{i,S}$ where $\Delta=N^{O(1/t)}$.
\item For all $i\ge0$, we have $|A_{i}|\le|\deg_{G}|/N^{i/t}$. In particular, $|A_{2t}|=0$. For all $i\ge1$, we have $|B_{i}|\le2|\deg_{G}|/N^{(i-1)/t}$.
\item \label{enu:total cap}$|\deg_{G'}|\le4t\Delta\omega|\deg_{G}|$.
\item \label{enu:edge len cap}For all $e\in E(G')$, $\ell_{G'}(e)=h$ and $u_{G'}(e)\in\frac{1}{h}\mathbb{Z}_{>0}$. 
\end{enumerate}
\end{prop}

\begin{proof}
(1): We assume that $A_{0}$ is integral. For $i\ge1$, $C_{i}(e)$ is a non-negative multiple of $\frac{1}{h_{\diam}s_{\decomp}}$ for all $e$ as $C_{i}$ is a $(h_{\diam}s_{\decomp})$-length moving cut. By induction, $A_{i}(v)$ and $B_{i}(v)$ are non-negative multiples of $\frac{\beta}{h_{\diam}s_{\decomp}}=\frac{1}{h}$. 

(2): By \ref{lem:router expander} and (1), we have $\deg_{H_{i,S}}\le(h|B_{i,S}|)^{O(1/t)}\cdot B_{i,S}$ since $B_{i}(v)\in\frac{1}{h}\mathbb{Z}_{>0}$. The bound on $\Delta$ follows using the trivial bound $|B_{i,S}|\le N^{O(1)}$.

(3): For $i=0$, this holds by the assumption. For $i\ge1$, we have that $|C_{i}|\le\kappa_{\decomp}\phi|A_{i-1}|$ by \ref{def:linked decomp} and so 
\[
|A_{i}|\le\beta|\deg_{C_{i}}|=2\beta|C_{i}|\le2\beta\kappa_{\decomp}\phi|A_{i-1}|\le|A_{i-1}|/N^{1/t}\le N^{1-i/t}
\]
by the choice of $\phi$ and by induction hypothesis. Since we have $|A_{2t}|\le N^{1-2t/t}<\frac{1}{h}$, it follows that $|A_{2t}|=0$ by (1).

(4): We have $|B_{i}|=|A_{i-1}|+\beta|A_{i}|\le2|\deg_{G}|/N^{(i-1)/t}$ by (3). 

(5): By (2) and the definition of neighborhood cover, we have $\sum_{S\in\cluster(\N_{i})}|\deg_{H_{i,S}}|\le\Delta\cdot\sum_{S\in\cluster(\N_{i})}|B_{i,S}|\le\Delta\omega2|\deg_{G}|/N^{(i-1)/t}$ . Since, $G'=\bigcup_{i\le2t}\bigcup_{S\in\cluster(\N_{i})}H_{i,S}$, we have $|\deg_{G'}|\le4t\Delta\omega|\deg_{G}|$.

(6): For each $e\in E(G')$, we have $\ell_{G'}(e)=h$ by construction and $u_{G'}(e)\in\frac{1}{h}\mathbb{Z}_{>0}$ because $B_{i}(v)\in\frac{1}{h}\mathbb{Z}_{\ge0}$ and by \ref{lem:router expander}. 
\end{proof}
\begin{comment}
%
\begin{prop}
\label{prop:emu bound edge}$|E(G')|\le n\cdot(t\omega)$.
\end{prop}

\begin{proof}
We gave $|\deg_{G'}|\le|\deg_{G}|\cdot N^{O(1/t)}\log N$.
\begin{itemize}
\item For each level $t$.
\begin{itemize}
\item For each clustering $\S\in\N_{i}$: $\omega=N^{O(1/t)}\log N$
\begin{itemize}
\item For each node in a router $\Delta\deg_{G}(u)$ where $\Delta\le N^{O(1/t)}$
\end{itemize}
\end{itemize}
\end{itemize}
\end{proof}
\end{comment}

We show that any demand in $G$ can be routed in $G'$ with small congestion, length, and steps. This is the key technical lemma and we defer the proof to \ref{sec:emu proof forward map}.
\begin{lem}
[Forward Mapping]\label{lem:forward map}Let $F$ be a flow in $G$ where $\congest_{F}=1$ and $\leng_{F}\le h$. There is a flow $F'$ routing $D_{F}$ in $G'$ with $\congest_{F'}\le\kappa_{\rt}$, $\leng_{F'}\le O(t\cdot t_{\rt}h)$, and $\step_{F'}\le O(t\cdot t_{\rt})$.
\end{lem}

Next, we show that the edge-demand in $G'$, which is the ``hardest demand'' by \ref{prop:edge demand}, can be routed in $G$ with small congestion and length. Roughly speaking, this is because the edge-demand in $G'$ in the ``$i$-th level'' is $B_{i}$-respecting but $B_{i}$ is expanding in $G$ by our construction.
\begin{lem}
[Backward Mapping]\label{lem:backward map}Let $D_{E(G')}$ be the edge-demand of $G'$ and let $F'$ be the canonical flow for $D_{E(G')}$. There exists a flow $F$ in $G$ that routes $D_{E(G')}$ where $\congest_{F}\le O(\omega t\cdot\Delta\phi^{-1}\log(N))$ and $L_{F}\preceq(h_{\diam}s_{\decomp}/h)\cdot L_{F'}$.
\end{lem}

\begin{proof}
Consider the neighborhood cover $\N_{i}=\{\S_{i,j}\}_{j=1}^{\omega}$ from \ref{alg:emu}. For each $i,j$, define 
\[
E'_{i,j}=\bigcup_{S\in\cluster(\S_{i,j})}\router(\deg_{S},t_{\rt},\kappa_{\rt}).
\]
Observe that $\{E'_{i,j}\}_{j}$ partitions the edge set $E'_{i}$ and $G'=\dot{\bigcup}_{i,j}E'_{i,j}$. Let $D'_{i,j}$ be the demand such that $D'_{i,j}(v,w)=D_{E(G')}(v,w)$ for each $(v,w)\in E'_{i,j}$, otherwise $D'_{i,j}(v,w)=0$. Let $F'_{i,j}$ be the subflow of $F'$ routing $D'_{i,j}$. Note that $D_{E(G')}=\sum_{i,j}D'_{i,j}$ and $F'=\sum_{i,j}F'_{i,j}$. We claim that there is a flow $F_{i,j}$ in $G$ routing $D'_{i,j}$ such that $\congest_{F_{i,j}}\le O(\Delta\phi^{-1}\log(N))$ and $L_{F_{i,j}}\preceq(h_{\diam}s/h)\cdot L_{F'_{i,j}}$. Assuming this, we define $F=\sum_{i,j}F_{i,j}$. Since $i$ ranges from $1\le i\le2t$ and $j$ ranges from $1$ to $\omega$, the congestion of $F$ blows up by $O(\omega t)$ factor, i.e., $\congest_{F}\le O(\omega t\cdot\Delta\phi^{-1}\log(N))$. By \ref{prop:len decompose}, we can bound the length of $F$ as $L_{F}\preceq(h_{\diam}s_{\decomp}/h)\cdot L_{F'}$.

Now we prove the claim. Fix $i$ and $j$. Each demand pair $(v,w)$ in $D'_{i,j}$ corresponds to an edge $(v,w)\in E'_{i,j}$. By definition of $\N_{i}$, we have that $\dist_{G-C_{i}}(v,w)\le h_{\diam}$. Also, $\sum_{w}D'_{i,j}(v,w)\le\deg_{E'_{i,j}}(v)\le\Delta B_{i}(v)$ by the guarantee of $\router(B_{i,S},t_{\rt},\kappa_{\rt})$ from \ref{lem:router expander} and the fact that each cluster $S\in\cluster(\S_{i,j})$ are vertex disjoint. That is, we have $\frac{1}{\Delta}D'_{i,j}$ is a $B_{i}$-respecting $h_{\diam}$-length demand in $G-C_{i}$. 

By definition, since $C_{i}$ be a $\beta$-linked $(h_{\diam},s_{\decomp},\phi,\kappa_{\decomp})$-decomposition for $A_{i-1}$, we have that $B_{i}=A_{i-1}+\beta\deg_{C_{i}}$ is $(h_{\diam},s_{\decomp})$-length $\phi$-expanding in $G-C_{i}$. So, by \ref{thm:flow character}, $\frac{1}{\Delta}D'_{i,j}$ can be routed in $G-C_{i}$ with congestion $O(\phi^{-1}\log(N))$ and length $h_{\diam}s_{\decomp}$. So $D'_{i,j}$ can be routed in $G$ via some flow $F_{i,j}$ with congestion $\congest_{F_{i,j}}\le O(\Delta\phi^{-1}\log(N))$ and length $\leng_{F_{i,j}}\le h_{\diam}s_{\decomp}$. Since $\leng_{F'_{i,j}}\ge h$ because every edge in $G'$ has length at least $h$, we have $L_{F_{i,j}}\preceq(h_{\diam}s/h)\cdot L_{F'_{i,j}}$ by \ref{fact:flow len all paths}.
\end{proof}
%
Combining the two key lemmas above, we conclude the following:
\begin{cor}
\label{lem:len emu guarantee}Let $G'=\textsc{Emulator}(G,t,h)$ be the output of \ref{alg:emu}. Then, $G'$ is a $O(t^{2})$-step $h$-length emulator for $G$ with length slack $(O(t^{2}),O(t^{2}))$ and congestion slack $(O(t),\poly(t)N^{O(1/t)})$. 
\end{cor}

\begin{proof}
By \ref{lem:forward map}, for any flow $F$ in $G$ where $\leng_{F}\le h$, there is a flow $F'$ routing $D_{F}$ in $G'$ with $\congest_{F'}\le\kappa_{1}\cdot\congest_{F}$ and $\leng_{F'}\le s_{1}\cdot h$ and $\step_{F'}\le O(t\cdot t_{\rt})$ where $\kappa_{1}=\kappa_{\rt}$ and $s_{1}=O(t\cdot t_{\rt})$. Combining \ref{prop:edge demand} and \ref{lem:backward map}, for any flow $F'$ in $G'$, there exists a flow $F$ in $G$ that routes $D_{F'}$ where $\congest_{F}\le\kappa_{2}\cdot\congest_{F'}$ and $L_{F}\preceq s_{2}\cdot L_{F'}$ where $\kappa_{2}=O(\omega t\cdot\Delta\phi^{-1}\log(N))$ and $s_{2}=(h_{\diam}s_{\decomp}/h)$.

Recall that we set $t_{\rt}=t$ and $\kappa_{\rt}=O(t)$. So $\kappa_{1}=O(t)$ and $s_{1}=O(t^{2})$. Also since $h_{\diam}=8th$ and $s_{\decomp}=t$, we have $s_{2}=O(t^{2})$. To calculate $\kappa_{2}$, we have $\omega=N^{O(1/t)}\log N$ by \ref{thm:cover basic} and and $\Delta=N^{O(1/t)}$ by \ref{lem:router expander}. Also, $\phi^{-1}=2\beta\kappa_{\decomp}N^{1/t}=\Otil(t^{2}N^{O(1/t)})$ because $\kappa_{\decomp}=N^{O(1/t)}\log N$, $\beta=h_{\diam}s_{\decomp}/h=O(t^{2})$. So $\kappa_{2}=\poly(t)N^{O(1/t)}$.
\end{proof}
With \ref{lem:len emu guarantee} above, \ref{thm:h leng emu} and \ref{thm:emu} are almost immediate except that we need to small points about the bounds of the length and capacity of edges in $G'$.

\paragraph{Proof of \ref{thm:h leng emu}.}

Suppose $\l_{G}(e),u_{G}(e)\in\mathbb{Z}_{>0}$ for all $e\in E(G)$. For all $e\in E(G')$, we have $\l_{G}(e)=h$ and $u_{G}(e)\in\frac{1}{h}\mathbb{Z}_{>0}$ by \ref{prop:basics}(\ref{enu:edge len cap}). Also, $\sum_{e\in E(G')}u_{G'}(e)\le\sum_{e\in E(G)}u_{G}(e)N^{O(1/t)}$ by \ref{prop:basics}(\ref{enu:total cap}).

\paragraph{Proof of \ref{thm:emu}.}

By plugging \ref{lem:len emu guarantee} with $h=2^{i}$ for all $0\le i\le\left\lceil \log(\diam(G))\right\rceil $ into \ref{lem:emu reduc}, we obtain a $O(t^{2})$-step emulator $G'$ for $G$ with length slack $O(t^{4})$ and congestion slack $\poly(t)N^{O(1/t)}$. Again, we have $u_{G}(e)\in\frac{1}{h}\mathbb{Z}_{>0}$ and $\sum_{e\in E(G')}u_{G'}(e)\le\sum_{e\in E(G)}u_{G}(e)N^{O(1/t)}$. We also have that $\diam(G')\le O(t^{2})\cdot\diam(G)$ by \ref{lem:forward map}.

\subsection{Proof of \ref{lem:forward map}: Forward Mapping}

\label{sec:emu proof forward map}

\paragraph{Strategy.}

Our strategy is to construct the flow $F'$ that routes $D_{F}$ in $G'$ incrementally. More concretely, let $D_{0}=D_{F}$. For each $i\ge1$, we will construct a flow $F'_{i}$ that partially routes $D_{i-1}$ in $G'$ using only edges from $E'_{i}$ so that the remaining demand is $D_{i}$. We maintain the invariant that, for all $i\ge0$, the demand $D_{i}$ is $A_{i}$-respecting and it is routable in $G$ with congestion $1$ and length $h$. (The set $A_{i}=\beta\deg_{C_{i}}$ is defined in \ref{alg:emu}.) 

By combining and concatenating these flows $F'_{i}$ for all $i\ge1$, we will obtain $F'$ with the desired properties. First, note that the invariant holds for $i=0$ since $\congest_{F}=1$ and $\leng_{F}\le h$ by assumption. Also, $D_{F}$ must be $A_{0}$-respecting because $A_{0}=\deg_{G}$ and $\congest_{F}=1$. For $i\ge1$, assuming that the invariant holds for $i-1$, we will construct the flow $F'_{i}$ that partially routes $D_{i-1}$ so that the invariant holds for $i$. 

\paragraph{Construct $F'_{i}$.}

The high-level idea is that we try to send a packet from $v$ to $w$ for each demand pair $(v,w)$ of $D_{i-1}$. If $\dist_{G-C_{i}}(v,w)\le h_{\cov}$, then we will successfully route this packet via some router and be done with it. Otherwise, $\dist_{G-C_{i}}(v,w)>h_{\cov}$. In this case, for each $(v,w)$-flow path $P$, we will identify a set of vertices $X_{v,P}$ and fractionally route the packet from $v$ to $X_{v,P}$. Similarly, the packet $w$ is routed to a set $X_{w,P}$ that we carefully define. We think of $v$ ``forward'' the packet to $X_{v,P}$ and $w$ ``forward'' the packet to $X_{w,P}$. The demand between $X_{v,P}$ and $X_{w,P}$ will induce the demand $D_{i}$ in the next level. Below, we explain this high-level idea in detail.

For each demand pair $(v,w)$ of $D_{i-1}$ where $\dist_{G-C_{i}}(v,w)\le h_{\cov}$, there must exist a cluster $S\in\cluster(\N_{i})$ where $v,w\in S$. We \emph{assign} the pair $(v,w)$ to such arbitrary cluster $S$. For each cluster $S\in\cluster(\N_{i})$, we route in $G'$ all demands $D_{i-1}(v,w)$ for all pairs $(v,w)$ assigned to $S$ using the edges of $\router(\deg_{S},t)$. Let $F_{S}^{\done}$ denote the flow in $G'$ between vertices in $S$ induced by the above routing. Let $D_{S}^{\mathrm{done}}$ be the demand routed by $F_{S}^{\done}$.

Now, we take care of the remaining demand pairs $(v,w)$ of $D_{i-1}$ where $\dist_{G-C_{i}}(v,w)>h_{\cov}=4h$. Let $F_{i-1}$ be a flow routing $D_{i-1}$ in $G$ with congestion $1$ and length $h$, whose existence is guaranteed by the invariant. Consider any $(v,w)$-flow-path $P$ of $F_{i-1}$. Since $\dist_{G-C_{i}}(v,w)>4h$ but $\l_{G}(P)\le\leng_{F_{i-1}}\le h$, $C_{i}$ must increase the length $P$ by least $3h$. Recall that the length increase on edge $e$ by $C_{i}$ is $C_{i}(e)h_{\diam}s_{\decomp}$ as $C_{i}$ is a $(h_{\diam}s_{\decomp})$-length moving cut. 

Let $E_{v,P}$ the edge set in $P$ closest to $v$ such that the total length increase by $C_{i}$ is at least $h$, i.e., $\sum_{e\in E_{v,P}}C_{i}(e)h_{\diam}s_{\decomp}\ge h$. Next, we define the vertex set $X_{v,P}\subseteq P$ as follows. For each $(x,y)\in E_{v,P}$ where $x$ is closer to $v$, include $x$ into the set $X_{v,P}$. Let us denote $e_{x}=(x,y)\in E_{v,P}$ as the edge corresponding to $x\in X_{v,P}$. Observe that, for any $x\in X_{v,P}$,
\[
\dist_{G-C_{i}}(v,x)\le\l_{G}(P)+h\le2h\le h_{\cov}
\]
That is, $X_{v,P}\subseteq\ball_{G-C_{i}}(v,h_{\cov})$ and so there exists a cluster $S\in\cluster(\N_{i})$ containing both $v$ and $X_{v,P}$. For each $x\in X_{v,P}$, we route flow in $G'$ from $v$ to $x$ of value at most 
\[
F_{i-1}(P)\cdot\frac{C_{i}(e_{x})h_{\diam}s_{\decomp}}{h}
\]
via $\router(B_{i,S},t_{\rt},\kappa_{\rt})$. Since $\sum_{x\in X_{v,P}}C_{i}(e_{x})h_{\diam}s_{\decomp}\ge h$ by definition, we can route flow from $v$ to $X_{v,P}$ of total value $F_{i-1}(P)$. Symmetrically, we define $E_{w,P}$ and $X_{w,P}$ . Observe that $X_{v,P}$ and $X_{w,P}$ are disjoint because they are defined based on vertices closest to $v$ and $w$, respectively. We route flow in $G'$ from $w$ to $X_{w,P}$ of total value $F_{i-1}(P)$ via $\router(B_{i,S},t_{\rt},\kappa_{\rt})$ where $S\in\cluster(\N_{i})$ is a cluster containing both $w$ and $X_{w,P}$.
\begin{comment}
Let $x_{v}$ be the vertex in $P$ closest to $v$ where $\deg_{C_{i}}(x_{v})>0$. Let $P_{v}$ denote the subpath of $P$ from $v$ to $x_{v}$. By the choice of $x_{v}$, $C_{i}$ cannot increase the length of any edge in $P_{v}$ and so $\dist_{G-C_{i}}(v,x_{v})\le\l_{G}(P_{v})\le h=h_{\cov}$. So there exists a cluster $S\in\cluster(\N_{i})$ containing both $v$ and $x_{v}$. We route in $G'$ from $v$ to $x_{v}$ with value $F_{i-1}(P)$ via $\router(B_{i,S},t_{\rt},\kappa_{\rt})$. Symmetrically, we define $x_{w}$ and $P_{w}$. 

Then, we route in $G'$ from $w$ to $X_{w,P}$ in the symmetric way.
\end{comment}
{} 

For each cluster $S\in\cluster(\N_{i})$, let $F_{S}^{\forward}$ be the flow in $G'$ induced by the routing described above, which routes from vertices with positive demand in $D_{i-1}$ to the vertices incident to the cut $C_{i}$. Let $D_{S}^{\forward}$ be the demand routed by $F_{S}^{\forward}$.

Finally, we define the flow $F'_{i}=\sum_{S\in\cluster(\N_{i})}F_{S}^{\done}+F_{S}^{\forward}$ in $G'$ that routes $D_{S}^{\mathrm{done}}$ and $D_{S}^{\mathrm{forward}}$ for all $S\in\cluster(\N_{i})$ in the manner described above.

\paragraph{$D_{S}^{\mathrm{done}}$ and $D_{S}^{\mathrm{forward}}$ are $B_{i,S}$-respecting.}

Here, we argue that both $D_{S}^{\mathrm{done}}$ and $D_{S}^{\mathrm{forward}}$ are $B_{i,S}$-respecting. This is useful because, by \ref{lem:router expander}, it means that both $D_{S}^{\mathrm{done}}$ and $D_{S}^{\mathrm{forward}}$ can be routed in $\router(B_{i,S},t_{\rt},\kappa_{\rt})\subseteq G'$ using $t_{\rt}$ steps and congestion $\kappa_{\rt}$. Since each edge in $G'$ has length $1$, the length of this routing is at most $t_{\rt}$. 

It suffices to show that $D_{S}^{\mathrm{done}}$ and $D_{S}^{\mathrm{forward}}$ are $B_{i}$-respecting because their supports are only on the pairs of vertices inside $S$. This is easy to argue for $D_{S}^{\mathrm{done}}$. We have $D_{S}^{\mathrm{done}}\le D_{i-1}$ (entry-wise), $D_{i-1}$ is $A_{i-1}$-respecting, and $A_{i-1}\le B_{i}$ (entry-wise). So $D_{S}^{\mathrm{done}}$ is $B_{i}$-respecting. Next, we analyze $D_{S}^{\mathrm{forward}}$. On one hand, the total demand that each vertex $v$ may send out is $\sum_{x}D_{S}^{\mathrm{forward}}(v,x)\le\sum_{x}D_{i-1}(v,x)\le A_{i-1}(v)$ because $D_{i-1}$ is $A_{i-1}$-respecting by the invariant. On the other hand, we claim that the total demand that each vertex $x$ may receive is $\sum_{v}D_{S}^{\mathrm{forward}}(v,x)\le\beta\deg_{C_{i}}(x).$ Since $B_{i}=A_{i-1}+\beta\deg_{C_{i}}$, we also have $D_{S}^{\mathrm{forward}}$ is $B_{i}$-respecting. 

Now, we prove the claim. The key observation is $\sum_{v}D_{S}^{\mathrm{forward}}(v,x)$ is at most 
\[
\sum_{e:\text{incident to }x}F_{i-1}(e)\frac{C_{i}(e)h_{\diam}s_{\decomp}}{h}.
\]
This is because, by construction of the flow $F_{S}^{\forward}$, $x$ may only receive the demand of quantity at most $F_{i-1}(P)\frac{C_{i}(e)h_{\diam}s_{\decomp}}{h}$ whenever $x\in P$ and $e\in P$ is incident to $x$. But we have

\[
\sum_{e:\text{incident to }x}F_{i-1}(e)C_{i}(e)\frac{h_{\diam}s_{\decomp}}{h}\le\sum_{e:\text{incident to }x}u_{G}(e)C_{i}(e)\beta=\beta\deg_{C_{i}}(x)
\]
because $F_{i-1}$ has congestion $1$ in $G$ and so $F_{i-1}(e)\le u_{G}(e)$. Also, $\beta=\frac{h_{\diam}s_{\decomp}}{h}$ by definition. This finishes the claim.

\paragraph{Define $D_{i}$ and Prove the Invariant.}

We define $D_{i}$ as the remaining demand after routing $F'_{i}$. Observe that the remaining demand is as follows. For each demand pair $(v,w)$ of $D_{i-1}$ where $\dist_{G-C_{i}}(v,w)>h_{\cov}$ and each $(v,w)$-flow-path $P$ of $F_{i-1}$, we need route flow of value from $X_{v,P}$ to $X_{w,P}$ of total value $F_{i-1}(P)$. Then, $D_{i}$ sums up these demand. 

Now, we argue that $D_{i}$ satisfies the invariant. Consider the congestion and length required for routing $D_{i}$ in $G$. Observe that $D_{i}$ only needs to route subpaths of the flow-paths of $F_{i-1}$ and $F_{i-1}$ is routable with congestion 1 and length $h$ in $G$. Therefore, $D_{i}$ is routable in $G$ with the same congestion and length bound.

Next, we show that $D_{i}$ is $A_{i}$-respecting. For $x\in\supp(A_{i})$, observe that the total demand that $x$ sends out in $D_{i}$ is the same as the total demand $x$ receives in $\sum_{S}D_{S}^{\mathrm{forward}}$. But we showed that this is at most $\sum_{e:\text{incident to }x}F_{i-1}(e)\frac{C_{i}(e)h_{\diam}s_{\decomp}}{h}\le\beta\deg_{C_{i}}(x)=A_{i}(x)$ by the definition of $A_{i}$. This completes the proof why the invariant holds. 

\paragraph{Construct $F'$ and Bound its Quality.}

The flow $F'$ is obtained by combining and concatenating the flows that route $D_{S}^{\mathrm{done}}$ and $D_{S}^{\mathrm{forward}}$ overall $S\in\cluster(\N_{i})$ for all level $i$ in a natural way so that $F'$ routes $D_{F}$. That is, in level $i$, each demand of $D_{i-1}$ is routed either successfully routed in $G'$ via some router in $t_{\rt}$ steps, or forwards to a new demand in $D_{i}$ by routing in $G'$ via some router in $t_{\rt}$ steps as well. As $i\le2t$, the maximum step of $F'$ is $O(t\cdot t_{\rt})$. Since the length of each edge of $G'$ is $h$, the length of $F'$ is at most $O(t\cdot t_{\rt}h)$. 

Now, we bound the congestion on $G'$. $F'$ simultaneously routes, for all $i$, $D_{S}^{\mathrm{done}}$ and $D_{S}^{\mathrm{forward}}$ for each $S\in\cluster(\N_{i})$ on $\router(B_{i,S},t_{\rt},\kappa_{\rt})$. Since $D_{S}^{\mathrm{done}}$ and $D_{S}^{\mathrm{forward}}$ are $B_{i,S}$-respecting, the congestion for routing both $D_{S}^{\mathrm{done}}$ and $D_{S}^{\mathrm{forward}}$ on $\router(B_{i,S},t_{\rt},\kappa_{\rt})$ is at most $\kappa_{\rt}$. But each router is edge-disjoint from each other, so the congestion for routing $F'$ on $G'$ is at most $\kappa_{\rt}$.

To summarize, we have successfully constructed a flow $F'$ routing $D_{F}$ in $G'$ with $\congest_{F'}\le\kappa_{\rt}$, $\leng_{F'}\le O(t\cdot t_{\rt}h)$, and $\step_{F'}\le O(t\cdot t_{\rt})$ as desired.

\begin{comment}

\subsection{Obliviousness}

\paragraph{Flow Mappings.}
\begin{definition}
[Flow Mapping]A multicommodity-flow mapping $\pi$ from a graph $G=(V,E)$ into a graph $G'=(V,E')$ takes a multicommodity flow $F$ in $G$ and assigns it a multicommodity flow $F'$ in $G'$ such that $D_{F'}=D_{F}$. We assume wlog that all multicommodity-flow mappings are linear, i.e., $\pi(\alpha F)=\alpha\pi(F)$.

We say $\pi$ is ($h$-length) $t$-hop if for every ($h$-length) flow $F$ in $G$, $\pi(F)(P)=0$ for any path $P$ in $G'$ with more than $t$ hops.

We say $\pi$ is ($h$-length) $\kappa$-congestion-preserving if for any ($h$-length) flow $F$ with congestion $1$ in $G$ the flow $F'=\pi(F)$ has congestion at most $\kappa$ in $G'$.

We say $\pi$ is ($h$-length) $s$-length-preserving if for any ($h$-length) flow $F$ in $G$ the flow $F'=\pi(F)$ in $G'$ satisfies that for all $u,v,l$ it holds that $L_{F'}(u,v,s\cdot l)\geq L_{F}(u,v,l)$.

We say $\pi$ is ($h$-length) $(s,\kappa)$-congestion-length-preserving if $\pi$ is both ($h$-length) $\kappa$-congestion-preserving and ($h$-length) $s$-length-preserving.
\end{definition}

\end{comment}



==> arxivver/import-lc-expander-prelims.tex <==
\section{Preliminaries}

\subsection{Graphs}

In this paper a graph $G$ is generally an undirected capacitated graph with integral positive length, integral positive capacities, at most one capacitated self-loop at any vertex. We use $V_G$ to denote the vertex set of $G$ and $n_G = |V_G|$ for the number of vertices. We use $E_G \subseteq \binom{V}{2}$ for the edge set and $m_G =|E|$ for the number of edges. We denote with $u_{G}:E\rightarrow\naturalnumbers$ the edge capacity function of $G$. The degree of a vertex $v$ is $\deg_{G}(v)=\sum_{(v,w)\in E}u_{G}(v,w)$. Note that a self-loop $(v,v)$ contributes $u_{G}(v,v)$ to the degree of $v$. We denote with $\l_{G}:E\rightarrow\naturalnumbers$ the edge length function of $G$.


We use standard graph terminology like adjacency, paths as sequences of edges, connectivity, connected components, etc. as defined in, e.g., \cite{west2001introGraph}. \\

{\bfseries Remark on Polynomially Bounded Object Sizes: }\\
All graphs and other objects defined in this paper are assumed to be of polynomial size in $n$, i.e., for any arbitrary but fixed constant $c_{\max}$ we assume that all objects are of size at most $N < n^{c_{\max}}$. In particular we only consider graphs\footnote{While our constructions and algorithms graphs sometimes grow an input graph or other objects a bit (e.g., by adding self-loops) such a growth is never by more than a polynomial factor overall.} with $m < N$. \enote{$m_g$?} This polynomial bound on object sizes in this paper also allows us to treat logarithmic upper bounds in the sizes of these objects as essentially interchangeable, e.g., for any constant bases $b,b'$ we have that $\log_b n \leq \log_b m_{\max} = \Theta(\log_{b'} N)$. Throughout the paper we therefore use $O(\log N)$ without any explicitly chosen basis to denote such quantities. It is understood that all $O$-notation depends on $c_{\max}$.


\subsection{(Normal) Expanders}

We use the following standard definition of a $\phi$-expander. If we want to emphasize that a graph is a $\phi$-expander in this standard sense and not a (length-constrained) $\phi$-expander we call such a $\phi$-expander a \emph{normal} $\phi$-expander.

\begin{definition}\label{def:normal-expander}
Given a graph $G=(V, E)$, for a set $S\subset V$, we define the sparsity of the cut $(S, V\setminus S)$ as $\frac{|E(S, V\setminus S)|}{\min\{\vol(S), \vol(V\setminus S)\}}$, where $\vol(T)=\sum_{v\in T} \degree(T)$ and $E(S, V\setminus S)$ denotes the set of edges that have exactly one endpoint in $S$. The conductance of graph is the smallest sparsity of any cut $(S, V\setminus S)$. A graph is a $\phi$-expander if its conductance is at least $\phi$.
\end{definition}

\subsubsection{(Normal) Expander Pruning}
\begin{theorem}[Simplified Version of Theorem 1.3 of \citet{saranurak2019expander}]\label{thm:expPrun} Let $G = (V, E)$ be $\phi$-expanding with $m$ edges, let $D \subseteq E$ be a collection of edges and let $G' = (V, E \setminus D)$ be $G$ with $D$ deleted. Then there is a set $P \subseteq V$ such that:
\begin{enumerate}
    \item $G'[V \setminus P]$ is $\frac{\phi}{6}$-expanding;
    \item $\vol(P) \leq \frac{8}{\phi} \cdot |D|$.
\end{enumerate}
\end{theorem}



\subsection{Paths and Length}

A path from vertex $v$ to vertex $w$ is called a $(v,w)$-path. For any path $P$ we define the length of $P$ to be $\l_{G}(P)=\sum_{e\in E}\l_{G}(e)$, i.e., the sum of all edge lengths of $P$. We furthermore call the number of edges in a path $P$ the step-length or simply step of $P$ and denote it with $\step{P}=|P|$. The \emph{distance} between vertices $v$ and $w$ is $\dist_{G}(v,w)=\min_{P:(v,w)\text{-path}}\l_{G}(P)$. A \emph{ball} of radius $r$ around a vertex $v$ is $\ball_{G}(v,r)=\{w\mid\dist_{G}(v,w)\le r\}$.\\


{\bfseries Remark on hop vs. length vs. step-length: }\\
For graphs in which every edges has length $1$ the step-length and length of a path are identical. Prior works primarily used the length-bounded expanders in the context of such unit-length graphs and talked about $h$-hop paths. To avoid confusions and maximize consistency with this prior work we use the following naming throughout this paper. We  exclusively use $\step$ to denote the number of edges in a path as defined above and use the words ``hop'' and ``length'' interchangeably to refer to $\l{P}$. By convention we primarily use ''hop'' when either referring to prior work on $h$-hop expanders or when talking about the length in unit-length graphs. Whenever we want to emphasize that arbitrary length functions can be used we prefer to talk about $l$-length expanders. 


\subsection{(Length-Constrained) Multicommodity Flows}

A \emph{(multicommodity) flow} $F$ in $G$ is a function that assigns simple paths $P$ in $G$ a flow value $F(P)\ge0$. We say $P$ is a \emph{flow-path} of $F$ if $F(P)>0$. $P$ is a \emph{$(v,w)$-flow-path} of $F$ if $P$ is both a $(v,w)$-path and a flow-path of $F$. The
$(v,w)$-flow $f_{(v,w)}$ of $F$ is such that $f_{(v,w)}(P)=F(P)$ if $P$ is a $(v,w)$-path , otherwise $f_{(v,w)}(P)=0$. The \emph{value}
of $f_{(v,w)}$ is $\val(f_{(v,w)})=\sum_{P\text{ is a }(v,w)\text{-path}}F(P)$. The value of $F$ is $\val(F) = \sum_{P} F(P)$.

The \emph{congestion of $F$ on an edge $e$} is $\congest_{F}(e)=F(e)/u_{G}(e)$
where $F(e)=\sum_{P:e\in P}F(P)$ denotes the total flow value of all paths going through $e$. The \emph{congestion} of $F$ is $\congest_{F}=\max_{e\in E(G)}\congest_{F}(e)$.
The \emph{length} of $F$, denoted by $\length_{F}=\max_{P:F(P)>0}\ell(P)$,
measures the maximum length of all flow-paths of $F$. The \emph{(maximum) step} of $F$ is $\step_{F}=\max_{P:F(P)>0}|P|$, which measures the maximum number of edges in all flow-paths of $F$. We sometimes write $\congest_{G,F},\length_{G,F},\step_{G,F}$ to emphasize that they are with respect to $G$.

\enote{Is $F(u,v)$, the flow between 2 vertices defined anywhere?}

\subsection{Demands and Node-Weightings}
All demands in this paper are directed, non-negative, and real-valued demands between nodes.

A \emph{demand} $D:V\times V\rightarrow\mathbb{R}_{\ge0}$ assigns
an non-negative value $D(v,w) \ge 0$ to each ordered pair of vertices. The size of a demand is written as $|D|$ and defined as $\sum_{v,w} D(v,w)$. Given a flow $F$, the \emph{demand routed/satisfied by $F$} is denoted
by $D_{F}$ where, for each $u,v\in V$,\emph{ }$D_{F}(u,v)=\sum_{P\text{ is a }(u,v)\text{-path}}F(P)$
is the value of $(u,v)$-flow of $F$. We say that a \emph{demand $D$ is routeable in $G$ with congestion $\eta$, dilation $h$, and
$t$} \emph{steps }if there exists a flow $F$ in $G$ where $D_{F}=D$, $\congest_{F}\le\eta$, $\length_{F}\le h$, and $\step_{F}\le t$. We say that an $\alpha$ fraction of $D$ is routeable if there exists a flow $F$ with $\val(F) \geq \alpha \cdot |D|$. \enote{Can't be any flow; should be one routing the input demand; easier if we define things in terms of sub-demands and then argue they're large and routable}


\enote{Can we force node weightings to never assign more than degree to a node?}
A \emph{node-weighting} $A:V\rightarrow\mathbb{R}_{\ge0}$ of $G$ assigns a value $A(v)$ to a vertex $v$. The \emph{size} of $A$ is denoted by $|A|=\sum_{v}A(v)$. 

DEFINE THE DEGREE NODE-WEIGHTINGS FOR (CAPACITATED) EDGE SETS, FOR MOVING CUTS (OR DO THIS LATER?), AND FOR A GRAPH G (SIMPLY THE NODE-WEIGHTING OF ALL THE GRAPHS EDGES). %For any moving cut $C$, the \emph{degree with respect to $C$} of a vertex $v$ is defined as 
%\[
%\deg_{C}(v)=\sum_{e\text{ incident to }v}u(e)\cdot C(e).
%\]

The load of a demand $D$, denoted with $\load{D}$, is the node-weighting which assigns the node $v$ the weight $\max\{\sum_{w \in V}D(v,w),\sum_{w \in V}D(w,v)\}$.

For two node-weightings $A,A'$ we define $\min{A,A'}$, $A-A'$, $A+A'$ as pointwise operations. We write $A \prec A'$ if $A$ is pointwise smaller than $A'$.

We say $D$ is \emph{$A$-respecting} if $\load{D} \prec A$. We say that $D$ is \emph{degree-respecting} if $D$ is $\deg_{G}$-respecting. A demand $D$ is called \emph{$h$-length-bounded }(or simply \emph{$h$-length} for short) if it assigns positive values only to pairs that are within
distance at most $h$, i.e., $D(v,w)>0$ implies that $\dist_{G}(v,w)\le h$. We call a demand integral if all $D(v,w)$ are integers and empty if $|D|=0$.

 




\mathversion{bold}
\subsection{$h$-hop Moving Cuts, $h$-hop Separation, and $h$-hop Sparsity}
\mathversion{normal}

\begin{definition}[$h$-length (moving) cut~\cite{networkcodinggap}]\label{def:movingcut}
An $h$-length moving cut $C: E \mapsto \{0,\frac{1}{h},\frac{2}{h},\dots,1\}$ assigns to each edge $e$ a fractional cut value between zero and one which is a multiple of $\frac{1}{h}$. The \emph{size} of $C$ is defined
as $|C|=\sum_{e}u(e)\cdot C(e)$. The length increase associated with the $h$-length moving cut $C$ is denoted with $\l_{C,h}$ and defined as assigning an edge $e$ the length $\l_{C,h}(e) = h\cdot C(e)$. Any moving cut which
only assigns cut values equal to either $0$ or $1$ is called a pure moving cut. 
\end{definition}

\begin{definition}[$G-C$]
For a graph $G$ with length function $l_G$ we denote with $G-C$ the graph $G$ with length function $l_{G-C} =  l_G + \l_{C,h}$. We refer to $G-C$ as the \emph{graph $G$ after cutting}
$C$ or \emph{after applying the moving cut} $C$.
\end{definition}


\begin{definition}[$h'$-hop separation]
Let $C$ be an $h'$-hop moving cut. We say two node $v,v' \in V$ are $h'$-hop separated by $C$ if their distance in $G-C$ is larger than $h$, i.e., if $\dist_{G-C}(v,v')>h$.
\end{definition}

\begin{definition}[$h'$-hop separated demand]
For any demand $D$ and any $h'$-hop moving cut $C$ we define the amount of $h'$-hop separated demand as the sum of demands between vertices that are $h'$-hop separated by $C$. We denote this quantity with $\sep_{h'}(C,D)$,
i.e., $$\sep_{h'}(C,D) = \sum_{e,e' \text{ with } \dist_{G-C}(e,e')>h'} D(e,e').$$
\end{definition}

\begin{definition}[$h'$-hop sparsity of a cut $C$ for a demand $D$]
For any demand $D$ and any $h'$-hop moving cut $C$ with $\sep_{h'}(C,D)>0$ the $h'$-hop sparsity of $C$ with respect to $D$ is the size of $C$ divided by the amount of demand $h'$-hop separated by $C$, i.e., 
$$\spa_{h'}(C,D) = \frac{|C|}{\sep_{h'}(C,D)}.$$
\end{definition}


Note that if a demand $D$ has any demand between vertices that have hop-distance exceeding $h'$ then the empty cut has an $h'$-hop sparsity for $D$ which is equal to zero. For all other demands, i.e., for any non-empty $h$-hop demand $D$ with $h \leq h'$, the $h'$-hop sparsity of any cut $C$ for $D$ is always strictly positive. We define the $h'$-hop sparsity of any $h'$-hop moving cut $C$ for a demand $D$ to be $\infty$ if $\sep_{h'}(C,D)=0$. This includes the empty cut.

\begin{definition}[$h'$-hop sparsity for a demand]
We say $C$ is a sparsest $h'$-hop cut for $D$ if $C$ minimizes $\spa_{h'}(C,D)$
among all $h'$-hop moving cuts $C'$. We say the demand $D$ has $h'$-hop sparsity $\phi$ if the sparsest $h'$-hop cut $C$ for $D$ has
$\spa_{h'}(C,D)=\phi$.
\end{definition}


\mathversion{bold}
\subsection{Hop-Slack, $(h,s)$-length Sparsity, $(h,s)$-length Conductance, and $(h,s)$-length $\phi$-Expanders}\label{sec:h-hop-expander-def}
\mathversion{normal}


\begin{definition}[$(h,s)$-length sparsity of a cut with respect to node-weighting]\label{def:sparsity}
The $(h,s)$-length sparsity of any $hs$-length moving cut $C$ with respect to a node-weighting $A$ is defined as:
$$\spa_{(h,s)}(C,A) = \min_{A\text{-respecting h-hop demand}\ D} \spa_{s \cdot h} (C,D)\enspace.$$
\end{definition}


\begin{definition}[$(h,s)$-hop conductance of a node-weighting]\label{def:conductance}
The $(h,s)$-length conductance of a node-weighting $A$ in a graph $G$ is defined as the $(h,s)$-length sparsity of the
sparsest $hs$-length moving cut $C$ with respect to $A$, i.e.,
$$\operatorname{cond}_{(h,s)}(A) = \min_{hs\text{ -length moving cut } C} \spa_{(h,s)}(C,A).$$ 
\end{definition}


When no node-weighting is mentioned then $(h,s)$-hop sparsity and $(h,s)$-length conductance are defined with respect to the $\deg_G$ node-weighting. I.e., the $(h,s)$-length sparsity of an $hs$-length moving cut $C$ in $G$ is defined as  $\spa_{(h,s)}(C,G) = \min_{\text{degree-respecting h-hop demand}\ D} \spa_{hs} (C,D)$ and the $(h,s)$-length conductance of a graph $G$ is defined as $\operatorname{cond}_{(h,s)}(G) = \min_{hs\text{ -length moving cut } C} \spa_{(h,s)}(C,\deg_G).$ 


\begin{definition}[$(h,s)$-hop $\phi$-expanders]
A graph $G$ is an $(h,s)$-hop $\phi$-expander if its $(h,s)$-hop conductance is at least $\phi$.
\end{definition}

\begin{definition}[$(h,s)$-hop $\phi$-expanding node-weightings]
We say a node-weighting $A$ is $(h,s)$-hop $\phi$-expanding in $G$ if the $(h,s)$-hop with respect to $A$ in $G$ is at least $\phi$. Equivalently we say $G$ is an $(h,s)$-hop $\phi$-expander for $A$.
\end{definition}

% \begin{lemma}[Observation after Definition 3.10 in \cite{haeupler2022hop}]
% For any integers $h' \leq h$ and any $\phi$ and $s$ if $A$ is $(h,s)$-hop $\phi$-expanding in $G$ then $A$ is also $(h', \frac{h}{h'} \cdot s)$-length $\phi$-expanding in $G$.
% \end{lemma}


\mathversion{bold}
\subsection{Relating Cut Sparsity, Expansion, and $h$-hop Min-Congestion}
\mathversion{normal}

\begin{theorem}\label{thm:sparse-cut-implies-congestion}
Suppose that for a demand $D$ there exists a $2h$-hop moving cut $C$ with $2h$-hop
sparsity $\phi = \spa_{2h}(C,D)$. Then, any $h$-hop routing of $D$ has
congestion at least $\frac{1}{2\phi}$.
\end{theorem}


\begin{theorem}\label{thm:flowcutgap}
Suppose that $D$ is a demand such that every $h$-hop moving cut $C$ has sparsity at
least $\phi$ for $D$, i.e., $\spa_{h}(C,D) \ge \phi$. Then, $D$ can be routed
along $h$-hop paths with congestion at most $O(\frac{\log n}{\phi})$.
\end{theorem}


\begin{corollary}\label{cor:flowcutgap}
In an $(h,s)$-hop $\phi$-expander any degree-respecting $h$-hop demand can be routed with congestion $O(\log n/\phi)$ along paths of length $O(s \cdot h)$.
\end{corollary}



% Combining \Cref{thm:sparse-cut-implies-congestion} and \Cref{thm:flowcutgap}
% directly gives \Cref{lem:expanders-routing-characterization} which shows that
% informally, and ignoring a logarithmic slack in the congestion and a constant
% slack in the dilation, $(h,s)$-hop $\phi$-expanders are exactly those graphs
% for which any $h$-hop demand $D$ can be routed over $\Theta(s \cdot h)$-hop
% paths with congestion $\tilde{\Theta}(\frac{\load(D)}{\phi})$.

% This is pretty much exactly what holds true in the non-hop-restricted setting where a graph is a $\phi$-expander if and only if every demand $D$ can be routed with congestion $\tilde{\Theta}(\frac{\load(D)}{\phi})$. This further justifies our choice of allowing non-pure cuts in our definitions.

\enote{Is the first point below different from the above corollary?}
\begin{lemma}\label{lem:expanders-routing-characterization}
For any $h \geq 1$, $\phi < 1$, and $s \geq 1$ we have that:\\
If $G$ is an $(h,2s)$-hop $\phi$-expander then any $h$-hop degree-respecting demand can be routed along $(2s \cdot h)$-length paths with congestion $O(\frac{\log N}{\phi})$.\\%[-0.3cm]
\noindent Conversely, if $G$ is not an $(h,2s)$-hop $\phi$-expander then some $h$-hop degree-respecting demand cannot be routed along $(s \cdot h)$-hop paths with congestion less than $\frac{1}{2\phi}$.
\end{lemma}


\begin{theorem}
[Flow Characterization of Hop-Constrainted Expanders (Lemma 3.16 of \cite{haeupler2022hop})]\label{thm:flow character}For any $h \geq 1$, $\phi < 1$, and $s \geq 1$ we have that:
\begin{enumerate}
\item If $A$ is $(h,s)$-length $\phi$-expanding in $G$, then every $h$-length $A$-respecting demand can be routed in $G$ with congestion at most $O(\log(N)/\phi)$ and length at most $s\cdot h$.
\item If $A$ is not $(h,s)$-length $\phi$-expanding in $G$, then some $h$-length $A$-respecting demand cannot be routed in $G$ with congestion at most $1/2\phi$ and dilation at most $\frac{s}{2}\cdot h$.
\end{enumerate}
\end{theorem}

%B: Look under Routers: An expander is a $O(log n/phi)$-step $O(log n/phi)$-router
%\enote{I need a lemma about routing in normal expanders a la the below; I just picked a hop slack that I assume is large enough:}
%\begin{lemma}[???]\label{lem:regExpEqualsHopExp}
%Suppose $G$ is a (normal) $\phi$-expander. Then $G$ is a $\left(\frac{\log N}{\phi}, 100 \right)$-hop $\phi$-expander.
%\end{lemma}


\subsection{Cut-Matching Games}\label{subsec:CutMatchingKRV}

Let $V$ be a set of vertices and let $A$ be a node-weighting with a strictly positive integer weight for every vertex in $V$. 

A cut-matching-game for $A$ with $r$ rounds
produces a sequence of graphs $G_0,\dots,G_r$ on the node set $V$ where $G_0$ is the empty graph. 

There are two players, the cut player and the matching player. 

In round $i$ the cut player chooses two integral node-weightings $A_i,B_i \preccurlyeq A$ of equal size and with disjoint support $S_i,T_i$ based on $G_i$. The cut player then produces a capacitated unit-length matching graph $G'_i=(V,M_i,u'_i)$ with edge set $M_i \subset S_i \times T_i$ and capacities $u'_i$ such that $deg_{G'_i} = A_i + B_i$. The graph $G_{i+1}$ is then simply $G_{i} + G'_i$, i.e., $G_{i+1}=(V,E_i,u_i)$ where $E_i = \bigcup_{j \leq i} M_j$ and $u_i = \sum_{j \leq i} u'_i$.

A cut strategy is a function which given a graph $G$ and node-weighting $A$ produces two node-weightings $A_i,B_i$ of nodes in $V_G$ with disjoint support. Similarly, a matching strategy is a function which given a graph $G$ and two node-weightings $A_i,B_i$ produces a valid matching graph $G_i$. 

We say a cut strategy is a $(r,t,\eta,\Delta)$-strategy for $A$ if the above game played for $r$ rounds against any matching strategy results in a graph $G_r$ which is a $t$-step $\eta$-congestion router for $A$ and for which $\deg{G_r} \preccurlyeq \Delta \cdot A$.
\enote{router not defined until later; what's the right order here?}


We say a cut strategy is a $(r,b,t,\eta,\Delta)$-batch-strategy if based on $G_i$ and $A$ not just one but $\ceil{r/b}$ node-weighting pairs $\{A_{i,j},B_{i,j}\}_{j\in[b]}$ are produced which the matching player gets to see and produce valid matching graphs for simultaneously. This results in $b$ batches. 

Note that if $A$ is a unit-weighting on vertex set $V$ then a cut player only selects the disjoint subsets $S_i,T_i \subset V$ of equal size and every valid matching graph $M_i$ has to be a unit-capacity perfect matching between $S_i$ and $T_i$.

\begin{claim}
\label{final cut matching game}
For every $A$ on some vertex set $V$ of size $n$ and every $t$ there exists an $(r,b,t,\eta,\Delta)$-batch-strategy with $r \leq t$ and $b,\eta,\Delta \leq n^{\poly(1/t)}$. This strategy can furthermore be efficiently computed (MAKE THIS MORE PRECISE). 
\end{claim}

DEFINE A NON-STOP VERSION AND/OR A MATCH PARTIALLY VERSION

\subsection{Hop-Constrained Expander Decomposition}

\begin{definition}
[Expander Decomposition]. An \emph{$(h,s)$-length $(\phi,\batch)$-expander
decomposition} for a node-weighting $A$ in a graph $G$ is a $(hs)$-moving
cut $C$ of size at most $\batch\phi|A|$ such that $A$ is $(h,s)$-length
$\phi$-expanding in $G-C$.
\end{definition}


\begin{definition}
[Linked Expander Decomposition]An \emph{$\beta$-linked $(h,s)$-length
$(\phi,\batch)$-expander decomposition} for a node-weighting $A$
in a graph $G$ is a $(hs)$-moving cut $C$ of size at most $\batch\phi|A|$
such that $A+\beta\cdot\deg_{C}$ is $(h,s)$-length $\phi$-expanding
in $G-C$. 
\end{definition}


We call $s$ and $\batch$ the length slack and congestion slack, respectively. We furthermore call an $\beta$-linked $(h,s)$-length $(\phi,\batch)$-expander
decomposition $C$ a $(h,s,\phi,\batch,\beta)$-decomposition for $A$, for short. Lastly, with an expander decomposition for a graph $G$ we simply mean an expander decomposition with for $\deg_G$ in $G$. 
We remark that an expander decomposition is simply a $\beta$-linked expander decomposition when $\beta=0$.


{\bfseries Remark: } It is convenient to require $\beta$ to be a multiple of $hs$ because in this case $\beta I_{C}$ is an integral node-weighting. 

\begin{theorem}
\label{thm:expdecomp exist} For any node-weighting $A$, length bound
$h$, length slack $s\ge100$, conductance bound $\phi>0$ there exists a $\beta$-linked $(h,s)$-length $(\phi,\batch)$-expander
decomposition for $A$ in $G$ with congestion
slack $\batch\le N^{O(1/s)}\log N$, and linkedness $\beta=\Omega(1/(\phi\log N))$. 
\end{theorem}
\begin{proof}
Follows from \cite{HopConstrainedExpanders1} except that one needs to scale the exponential demand in the potential analysis depending on $s$. For smaller $s$ one reduces the length of the exponential demand at the cost of an exponentially smaller overlap $h$-hop mixing leading to the larger $\batch$. CHECK THAT THIS LOSS DOES NOT APPLY TO $\beta$, TOO!
\end{proof}


\begin{claim}
\label{thm:expdecomp alg} For any $\eps > 0$ node-weighting $A$, length bound
$h$, length slack $s = 2^\Omega(\frac{1}{\eps})$, and conductance bound $\phi>0$ there exists an algorithm which deterministically in $n \poly\log N \cdot N^{\poly\eps}$ time computes a $\beta$-linked $(h,s)$-length $(\phi,\batch)$-expander
decomposition for $A$ in $G$ with congestion
slack $\batch\ge N^{O(\eps + 1/s)}\log N$, and linkedness $\beta=O(\frac{1}{\phi} \cdot \frac{1}{N^{eps}\log N})$.
\end{claim}


% \subsection{Routers}


% \begin{definition}[Routers]\label{def:router}
% A \emph{unit-length} capacitated graph $G$ is a $t$-step $\eta$-router for a node-weighting $A$ if every $A$-respecting demand can be routed in $G$ with $\eta$ congestion and $t$ steps.
% \end{definition}

% By the flow characterization of hop-constrained expanders \ref{thm:flow character},
% observe that routers are essentially the same object as length-constrained expanders when the graph has unit length and bounded diameter. 

% \begin{proposition}
% Let $G$ be a graph with unit edge-length. Let $A$ be a node-weighting where $\diam_{G}(\supp(A))\le h$.
% \begin{enumerate}
% \item If $G$ is a $(h,s)$-length $\phi$-expander for $A$, then $G$
% is a $(hs)$-step $O(\frac{\log N}{\phi})$-router for $A$.
% \item If $G$ is not a $(h,s)$-length $\phi$-expander for $A$, then $G$
% is not $(\frac{hs}{2})$-step $\frac{1}{2\phi}$-router for $A$. 
% \end{enumerate}
% \end{proposition}

% The following are examples of simple routers:
% \begin{example}
% Let $A$ be a node-weighting.
% \begin{enumerate}
% \item Let $H$ be a star where rooted at $r$ and the set of leaves is $\supp(A)$.
% The capacity of each star-edge $(r,v)\in E(H)$ is $A(v)$. Then,
% $H$ is a $2$-step $1$-router for $A$.
% \item Let $H$ be a complete graph where $V(H)=\supp(A)$. For each $v,w\in\supp(A)$,
% the capacity of $(v,w)$ is $\frac{A(v)\cdot A(w)}{|A|}$. Then, $H$
% is a $2$-step $2$-router for $A$. 
% \end{enumerate}
% \end{example}

% \begin{lemma}
% \label{lem:router hypercube}For any node-weighting $A$ where $a=|\supp(A)|$
% and a parameter $t$, there exists a $O(t)$-step $(a^{O(1/t)}\log a)$-router,
% denoted by $H=\router(A,\eps)$, such that 
% \begin{itemize}
% \item $V(H)=\supp(A)$, 
% \item $|E(H)|=a^{1+O(1/t)}\log a$,
% \item $\deg_{H}(v)=A(v)$ for all $v\in V(H)$.
% \end{itemize}
% \end{lemma}

\subsection{Neighborhood Covers}


Given a graph $G$ with lengths (or equivalently any metric on a vertex set $V$), a \emph{clustering} $\cS$ in $G$ with diameter $h_{\diam}$ is a collection of mutually
disjoint vertex sets $S_1,\ldots,S_{|\cS|}$, called clusters, where for every cluster has (weak) diameter at most $h_{\diam}$, i.e., $\forall i: \ \diam_{G}(S_i):=\max_{v,w\in U}\dist_{G}(u,v)\le h_{\diam}$. A clustering furthermore has absolute separation $h_{\sep}$ or separation-factor $s$ if the distance between any two clusters is at least $h_{\sep}$ or $s
\cdot h_{\diam}$, respectively. 

A neighborhood cover $\cN$ with width $\omega$ and covering radius $h_{\cov}$ is a collection of $\omega$ many clusterings $\cS_1, \ldots, \cS_\omega$ such that for every node $v$ there exists a cluster there exists an $i,j$ such that the cluster $\ball(v,h_{\cov}) \subseteq S_{i,j}$.

A neighborhood cover $\cN$ has diameter $h_{\diam}$ if every clustering has diameter at most $h_{\diam}$ and absolute separation $h_{\sep}$ or separation-factor $s$ if this applies to each of its clusterings. 

Lastly, we denote with $\load_{\cN}$ the maximum number of clusters (or clusterings) any node $v$ is contained in. 

%To eliminate an extra $\log n$ factor one can define the min cover frequency as the smallest number of times any neighborhood is covered and compare this to the load. We call this ratio the $\loadfactor_{\cN}$. 


\begin{theorem}
\label{thm:cover-separation-factor-existential}
For any $h_{\cov}, s, \eps, \eps'$ and graph $G$ there exists a neighborhood cover with covering radius $h_{\cov}$, separation-factor $s$, diameter $h_{\diam} = s^{1/\eps} \cdot \frac{1}{\eps'} \cdot h_{\cov}$, width $\omega = N^{O(\eps)} \log N$, $\load_{\cN} = N^{O(\eps')} \log N$.%, $\minload_{\cN} = \Omega(\log N)$.%,  $\loadfactor_{\cN} = N^{O(\eps')}$.
\end{theorem}



\begin{theorem}
\label{thm:cover-absolute-separation-existential}
For any $h_{\cov}, h_{\sep}, \eps, \eps'$ and graph $G$ there exists a neighborhood cover with covering radius $h_{\cov}$, separation $h_{\sep}$, diameter $h_{\diam} = \frac{h_{\sep}}{\eps \eps'} \cdot h_{\cov}$, width $\omega = \frac{N^{O(\eps)}}{\eps} \cdot \log N$, $\load_{\cN} = N^{O(\eps')} \log N$.%, $\minload_{\cN} = \Omega(\log N)$.%,  $\loadfactor_{\cN} = N^{O(\eps')}$.
\end{theorem}





\begin{theorem}
There exists a deterministic CONGEST algorithm
that given $h_{\cov}, \eps, \eps'$ and either a separation-factor $s$ or an absolute separation $h_{\sep}$ computes a neighborhood cover with the parameters provided in \Cref{thm:cover-separation-factor-existential} or \Cref{thm:cover-absolute-separation-existential}, respectively, in $h_{\diam} \cdot N^{O(\eps + \eps')}$ rounds and total work $\tO(n) \cdot \frac{N^{O(\eps + \eps')}}{\eps} \cdot h_{\diam}$. There also exists a deterministic PRAM algorithm with depths $\tO(N^{O(\eps + \eps')})$
and total work $\tO(n) \cdot N^{O(\eps + \eps')}$
and $h_{\diam} \cdot N^{O(\eps + \eps')}$ rounds.
\end{theorem}








\subsection{Hop-Constrained Cutmatches}

\begin{theorem}{mainThm}
\label{thm:main}
Given a digraph $D=(V,A)$ with capacities $u$, lengths $\l$, length constraint $h \geq 1$, $ \eps > 0$ and source and sink vertices $S, T \subseteq V$, one can compute a feasible $h$-length flow, moving cut pair $(f, C)$ that is $(1 \pm \epsilon)$-approximate in:
\begin{enumerate}
    \item Deterministic parallel time $\tilde{O}(\frac{1}{\eps^9} \cdot h^{17})$ with $m$ processors
    % \item Deterministic parallel time $\tilde{O}(h^{12})$ with $m$ processors;
    \item Randomized CONGEST time $\tilde{O}(\frac{1}{\eps^{9}} \cdot h^{17})$ with high probability;
    \item Deterministic CONGEST time $\tilde{O}\left(\frac{1}{\eps^9} \cdot h^{17}  + \frac{1}{\eps^7} \cdot h^{16} \cdot (\rho_{CC})^{10} \right)$.
\end{enumerate}
Also, $f = \eta \cdot \sum_{j=1}^k f_j$ where $\eta = \tilde{\Theta}(\epsilon^2)$, $k = \tilde{O}\left(\frac{h}{\epsilon^4} \right)$ and each $f_j$ is an integral $h$-length $S$-$T$ flow.
\end{theorem}

More generally than $\batch$ commodities, we solve the problem provided our commodities can be grouped into $\batch$ batches that are far apart.

\begin{definition}[$\batch$-Batchable]
 Given digraph $D$ with lengths $\l$ and source, sink set pairs $\{S_i, T_i\}_i$ we say that a $\{S_i, T_i\}_i$ is $\batch$-batchable if the pairs of $\{S_i, T_i\}_i$ can be partitioned into batches $\{\cS_j, \cT_j\}_j$ if 
 \begin{enumerate}
     \item For each $i$ there some $j$ such that $S_i \in \cS_j$ and $T_i \in \cT_j$;
     \item For each $i$ and $i'$, if $v \in S_i \cup T_i$ and $v' \in S_{i'} \cup T_{i'}$ and $S_i, S_{i'} \in \cS_j$ for some $j$ then $d_{\l}(v,v') > 2h$.
 \end{enumerate}
\end{definition}
Observe that if the number of commodities is $\batch$ then the set of source, sink pairs is trivially $\batch$-batchable.

The following summarizes our main result for computing multi-commodity length-constrained flows and moving cuts.
\begin{theorem}\label{thm:CutMatchAlgoMulti}
Given a digraph $D=(V,A)$ with capacities $u$, lengths $\l$, length constraint $h \geq 1$, $0 < \eps < 1$ and source and sink vertices $S, T \subseteq V$, and $\batch$-batchable source, sink pairs $\{S_i, T_i\}_i$, one can compute a feasible multi-commodity $h$-length flow, moving cut pair $(f, C)$ that is $(1 \pm \epsilon)$-approximate in:
\begin{enumerate}
    \item Deterministic parallel time $\tilde{O}(\batch \cdot \frac{1}{\eps^9} \cdot h^{17})$ with $m$ processors
    % \item Deterministic parallel time $\tilde{O}(h^{12})$ with $m$ processors;
    \item Randomized CONGEST time $\tilde{O}(\batch \cdot \frac{1}{\eps^{9}} \cdot h^{17})$ with high probability;
    \item Deterministic CONGEST time $\tilde{O}\left(\batch \cdot \frac{1}{\eps^9} \cdot h^{17}  + \batch \cdot \frac{1}{\eps^7} \cdot h^{16} \cdot (\rho_{CC})^{10} \right)$.
\end{enumerate}
Furthermore, $f = \eta \cdot \sum_{j=1}^k f_j$ where $\eta = \tilde{\Theta}(\epsilon^2)$, $k = \tilde{O}\left(\batch \cdot \frac{h}{\epsilon^4} \right)$ and $f_j$ is an integral $h$-length $S_i$-$T_i$ flow for some $i$.
\end{theorem}

In what follows, for a vertex subset $W \subseteq V$ we let $u^+(W) = \sum_{v \in W}\sum_{a \in \delta^+(v)}u_a$ and $u^-(W) = \sum_{v \in W} \sum_{a \in \delta^-(v)}u_a$. We also let $\delta^{\pm}(S,T) := \bigcup_{v \in S} \delta^+(v) \cup \bigcup_{v \in T} \delta^-(T)$

\begin{definition}[$h$-Length Cutmatch]\label{def:cutmatch}
Given digraph $D = (V,A)$ with capacities $u$ and lengths $\l$, an $h$-length $\phi$-sparse cutmatch of congestion $\gamma$ between two node sets $S,T \subseteq V$ with $u^+(S) \leq u^-(T)$ consists of:
\begin{itemize}
    % \item An out-node-weighting $w^+$ of $S$;
    % \item An in-node-weighting $w^-$ of $T$;
    \item An integral $h$-length $S$-$T$ flow $f$ in $D$ with capacities $\{u_a\}_{a \in \delta^{\pm}(S,T)} \cup \{\gamma \cdot u_a\}_{a \not \in \delta^{\pm}(S,T)}$;
    \item A moving cut $C$ of $S$ and $T$ in $D$ with capacities $\{u_a - f_a\}_{a \in \delta^{\pm}(S,T)} \cup \{u_a\}_{a \not \in \delta^{\pm}(S,T)}$ of value $ \sum_a C_a \leq \phi \cdot \left(u^+(S)-\val(f)\right)$.
\end{itemize}
\end{definition}

\begin{theorem}\label{lem:matchcut-old-purecut}
Suppose we are given a digraph $D = (V,A)$ with capacities $u$ and lengths $\l$. There is an algorithm that, given two node sets $S,T \subseteq V$ with $U^+(S) \leq U^-(T)$ and two integer parameters $h \geq 1$ and $\phi \leq 1$, outputs an $h$-length $\phi$-sparse cutmatch of congestion $\gamma$ between $S$ and $T$, where $\gamma=\tilde{O}(\frac{1}{\phi})$. This algorithm runs in:
\begin{enumerate}
    \item Deterministic parallel time $\tilde{O}(\gamma \cdot h^{18})$ with $m$ processors
    % \item Deterministic parallel time $\tilde{O}(h^{12})$ with $m$ processors;
    \item Randomized CONGEST time $\tilde{O}(\gamma \cdot h^{18})$ with high probability;
    \item Deterministic CONGEST time $\tilde{O}\left(\gamma \cdot h^{18}  + \gamma \cdot h^{17} \cdot (\rho_{CC})^{10} \right)$.
\end{enumerate}
\end{theorem}


TODO: change to $\batch$-batch







\subsection{Routers}
%\begin{itemize}
%\item Use $\kappa_{\mathrm{router}}$ and %$\kappa_{\mathrm{decomp}}$ instead.
%\end{itemize}
\enote{Should the following require that the node weightings are degree respecting or should we, alternatively, define node weights as never assigning a value larger than degree?}
Next, we define the notion of \emph{routers}.
\begin{definition}
[Routers]\label{def:router}For any node-weighting $A$, we say that
a \emph{unit-length} capacitated graph $G$ is a \emph{$t$-step $\eta$-router
for $A$} if every $A$-respecting demand can be routed in $H$ with
$\kappa$ congestion and $t$ steps.
\end{definition}

By the flow characterization of hop-constrained expanders \ref{thm:flow character},
observe that routers are essentially the same object as $(h,s)$-length $\phi$-expanders with unit length $t=\Theta(hs)$ long routing paths, congestion $\kappa = \tilde{\Theta}(\frac{1}{\phi})$ congestion, and a diameter smaller than $h$, which guarantees that any demand is $h$-length and therefore any degree-respecting demand must be routable. 

\begin{proposition}
Let $G$ be a graph with unit edge-length. Let $A$ be a node-weighting where $\diam_{G}(\supp(A))\le h$.
\begin{enumerate}
\item If $G$ is a $(h,s)$-length $\phi$-expander for $A$, then $G$
is a $(hs)$-step $O(\frac{\log N}{\phi})$-router for $A$.
\item If $G$ is not a $(h,s)$-length $\phi$-expander for $A$, then $G$
is not $(\frac{hs}{2})$-step $\frac{1}{2\phi}$-router for $A$. 
\end{enumerate}
\end{proposition}

\begin{proof}
Since $\diam_{G}(\supp(A))\le h$, the set of $A$-respecting demands
and the set of $h$-length $A$-respecting demands are identical.
Also, the notion of dilation and maximum steps of a flow in $G$ become
the same as edges have unit length. Therefore, by \ref{thm:flow character},
if $G$ is a $(h,s)$-length $\phi$-expander for $A$, then every
$A$-respecting demand can be routed in $G$ with congestion $O(\log(N)/\phi)$
and $sh$ steps. Otherwise, some $A$-respecting demand cannot be
routed in $G$ with congestion $1/2\phi$ and $(sh)/2$ steps. This
completes the proof by \ref{def:router}.
\end{proof}
%

\begin{example}\label{ex:routers}
Let $A$ be a node-weighting.
\begin{enumerate}
\item Let $H$ be a star where rooted at $r$ and the set of leaves is $\supp(A)$.
The capacity of each star-edge $(r,v)\in E(H)$ is $A(v)$. Then,
$H$ is a $2$-step $1$-router for $A$.
\item Let $H$ be a complete graph where $V(H)=\supp(A)$. For each $v,w\in\supp(A)$,
the capacity of $(v,w)$ is $\frac{A(v)\cdot A(w)}{|A|}$. Then, $H$
is a $2$-step $2$-router for $A$. 
\item If $H$ is a constant degree expander with constant conductance then $H$ is a $O(\log n)$-step $O(\log n)$-router and $H^k$ is a $O(\log n/k)$-step $O(\log n/k)$-router.
\end{enumerate}
\end{example}

\enote{Maybe should be a proof of this; fact that expanders mix can cite a survey; kth powergraph mixes k times faster}

%The router based on a star is sparse but it introduces new vertex
%not in $\supp(A)$. On the other hand, the router based on a complete
%graph is dense but uses only vertices in $\supp(A)$. It turns out
%that we can get the best of both worlds. 

Next we generalize the expander example to any node-weighting. 

\begin{lemma}\label{lem:router}
For any vertex set $V$, any $t$, and any integral node-weighting $A$ on $V$ there exists a $\Delta = |A|^{O(1/t)}$ and a $t$-step router $G$ with $\deg_G = \Delta \cdot A$ and congestion $O(\frac{\log |A|}{t})$.
\end{lemma}
\begin{proof}
Let $H$ be a $\Delta'$-regular expander with constant $\Delta'$ and constant conductance on a vertex set of size $|A|$. This is a $t'=O(\log |A|)$-router with congestion $O(\log |A|)$. Let $k = \ceil{\frac{t'}{t}}$. The graph $H^k$ is a $t$-hop router with congestion $\Theta(t)$ and regular degree $\Delta'^k$. Partitioning nodes of this graph into groups according to $A$ and contracting these groups results in the desired router. 
\end{proof}



% \subsection{Neighborhood Covers}
% \begin{itemize}
% \item $s_{\mathrm{decomp}}$ and $s_{\mathrm{cover}}$
% \item change from $U\in\cU$ to $S\in\S$ 
% \end{itemize}
% %
% Given a graph $G$, a \emph{clustering} $\cU$ in $G$ with diameter
% $h_{\diam}$ and separation factor $s$ is a collection of mutually
% disjoint vertex sets such that for each set $U\in\cU$, $\diam_{G}(U):=\max_{v,w\in U}\dist_{G}(u,v)\le h_{\diam}$
% and $\dist_{G}(U,U')\ge s\cdot\diam_{G}(U)$ for $U\neq U'\in\cU$.
% We call $\cU$ a \emph{$(h_{\diam},s)$-clustering} and each set $U\in\cU$
% a \emph{cluster}. 

% An \emph{$(h_{\cov},h_{\diam},s)$-neighborhood cover} $\N=\{\cU_{i}\}_{i=1}^{\omega}$
% of $G$ is a collection of $\omega=\mathrm{width}(\N)$ many \emph{$(h_{\diam},s)$}-clusterings
% in $G$ such that for each vertex $v$, there exists a cluster $U\in\cU_{i}$
% where $\ball(v,h_{\cov})\subseteq U$. We call $h_{\cov}$ a covering
% radius of $\N$ and $\omega$ the width of \textbf{$\N$}. Let $\cluster(\N)=\bigcup_{i=1}^{\omega}\cU_{i}$
% collect all clusters from each clustering $\cU_{i}$. We say that
% $\N$ is a \emph{$(h_{\cov},h_{\diam})$}-neighborhood cover when
% $s=0$, i.e., we only require all clusters in each clustering to be
% disjoint.
% \begin{itemize}
% \item Define the load of $v$ on $\N$ is : $\mathrm{load}_{\N}(v)=|\{\cU_{i}\mid v\in\cU_{i}\}|$
% \item $\mathrm{load}(\N)=\max_{v}\{\mathrm{load}_{\N}(v)\}$.
% \item Load ratio: $\textrm{load-ratio}(\N)$
% \item Width: $\omega=\mathrm{width}(\N)$
% \end{itemize}
% \begin{thm}
% \label{thm:cover}For any graph $G$, covering radius $h_{\cov}$,
% an integer $k\ge1$, there exists an $(h_{\cov},h_{\diam},o)$-neighborhood
% cover of $G$ with diameter $h_{\diam}\le(2k-1)h_{\cov}$ and overlapping
% parameter $o\le n^{1/k}\log n$.
% \end{thm}

% \begin{thm}
% \label{thm:cover sep}For any graph $G$, covering radius $h_{\cov}$
% and separation $h_{\sep}\ge??\cdot h_{\cov}$, an integer $k\ge1$,
% there exists an $(h_{\cov},h_{\diam},h_{\sep},o)$-neighborhood cover
% of $G$ with diameter $h_{\diam}\le??$ and overlapping parameter
% $o\le???$.
% \end{thm}

% \begin{itemize}
% \item CITE THIS.
% \begin{itemize}
% \item $h_{\diam}\le\frac{s^{O(1/\eps)}}{\eps'}\cdot h_{\cov}$
% \item $\load(\N)=n^{O(\eps')}\log n$
% \item $\width(\N)=n^{O(\eps)}\log n$
% \end{itemize}
% \end{itemize}
% %

==> arxivver/intro.tex <==


\section{Introduction}
\thatchaphol{Add discussion and citation to literature on hopset. Make citations up to date. Maybe add a discussion that about width reduction for Garg-Koennermann.}
In the maximum flow problem, we are given an edge-capacited graph $G=(V,E)$ and two vertices $s,t\in V$ with the aim to send as much flow as possible from $s$ to $t$. Maximum flow is a fundamental problem in combinatorial optimization with a long history, from the classic Ford-Fulkerson algorithm \cite{cormen2022introduction} to the recent breakthrough almost-linear time algorithm of Chen~et~al.~\cite{chen2022maximum}. The maximum flow problem also exhibits rich structural properties, most notably in the \emph{max-flow min-cut theorem}, which states that the value of the maximum flow between $s$ and $t$ is equal to the size of the minimum edge cut separating $s$ and $t$.

% Natural generalizations of maximum flow have also been well studied. 
A well-studied generalization of the maximum flow problem is the maximum \emph{multi-commodity flow} problem. Here, we are given $k\ge1$ pairs $(s_i,t_i)_{i\in[k]}$ of vertices and wish to maximize the amount of flow sent between each pair. %\footnote{There are two popular variants of multi-commodity flow, \emph{concurrent} and \emph{non-concurrent}. We study both in this paper, but for simplicity we will not distinguish between them in the introduction.}
On the algorithmic side, this problem can be solved in polynomial time by a linear program, and there has been exciting recent progress towards obtaining faster algorithms, both exact~\cite{van2023faster} and $(1+\epsilon)$-approximate~\cite{sherman2017area}. However, naively the best running time one can hope for is $O(mk)$, as even outputting the optimal solution may take $O(mk)$ time: each edge may carry flow from all $k$ commodities in a (near) optimal multi-commodity flow. Designing multi-commodity flow algorithms is further complicated by the loss of structure exhibited in the single-commodity setting. Specifically, the max-flow min-cut equality no longer holds in the multi-commodity case, and the flow-cut gap (i.e.\ the multiplicative difference between the max-flow and min-cut) is known to be $\Theta(\log n)$ for undirected graphs~\cite{leighton1999multicommodity} and $\Omega(n^{1/7})$ for directed graphs~\cite{chuzhoy2009polynomial}.

The algorithmic and structural issues above suggest that outputting a (near) optimal multi-commodity flow in time less than $O(mk)$ may be impossible. However, they leave open the possibility of efficiently approximating \emph{the value} of the optimal multi-commodity flow. Nonetheless, even for undirected graphs, standard techniques for optimal flow value approximation in the single-commodity setting fail to produce good approximation algorithms in the multi-commodity setting. For example, one natural approach that works in the single-commodity setting but not the multi-commodity setting is that of \emph{cut sparsifiers} \cite{benczur2015randomized,benczur1996approximating,li2021deterministic}. A cut sparsifier of a graph is a sparse (sub)graph with $\tilde O(n)$ edges that approximately preserve all cuts of the input graph. In the single-commodity setting, one can compute a $(1+\epsilon)$-approximate cut sparsifier, solve max-flow on the sparsifier, and return the value of this flow as an approximation to the optimal value in the original graph. However, because of the aforementioned flow-cut gap, this approach only achieves an approximation ratio of $O(\log n)$ in the multi-commodity setting.

\subsection{Our Results}
%In this paper, we break the $O(mk)$ barrier for estimating the optimal multi-commodity flow value on undirected graphs.

In this paper, we break the $O(mk)$-time barrier by giving $(m+k)^{1+\epsilon}$-time algorithms with constant-approximations to the value of the maximum $k$-commodity flow on undirected graphs for any constant $\eps > 0$.

% More formally,
We consider both concurrent and non-concurrent flow problems. 
In the concurrent flow problem, given a capacitated graph and a demand function, the goal is to find a maximum-value capacity-respecting flow routing a multiple of the demand. In the non-concurrent flow problem, given a capacitated graph and a set of vertex pairs, the goal is to find a maximum-value capacity-respecting flow routing flow only between vertex pairs in the given set. 

Our results can be informally summarized as follows:\thatchaphol{Check if there is other place that claim deterministic. Say that the only randomized place is ED}
%We give a constant approximation for the maximum value of a flow for both problems in close-to-linear time, breaking the $O(mk)$-flow decomposition barrier:
\begin{theorem}[Constant Approximate Concurrent/Non-Concurrent Flow (informal)]\label{thm:informal-constapprox-cnc-flow}
    For every constant $\epsilon \in (0, 1)$, there exists a $(m + k)^{1 + \poly(\eps)}$-time $O(2^{-1 / \eps})$-approximate algorithm for the concurrent and non-concurrent multicommodity flow value problems, where $k$ is the number of demand pairs. The algorithms work in parallel with depth $(m + k)^{\poly(\eps)}$. 
\end{theorem}

% \begin{quote}\centering
%     We give $O\left((m+k)^{1+\epsilon}\right)$ time algorithms which give constant-approximations to the value of the maximum $k$-commodity flow on undirected graphs for any constant $\eps > 0$.
% \end{quote}

% ADD CITATIONS FOR HOPSETS
The key to the above result is a powerful new tool we introduce called \emph{low-step (multi-commodity) flow emulators}. Informally, a low-step flow emulator of an undirected graph is another graph which contains approximate multi-commodity flows whose flow paths contain a small number of edges. Because they are not based on cuts, such emulators face no $\Omega(\log n)$ flow-cut barriers, unlike the above-mentioned cut sparsifiers. It is instructive to view low-step flow emulators as a generalization of \emph{hopsets}, which are graphs that contain approximate shortest paths of low step-length (but do not respect capacities). We additionally give efficient algorithms to construct these objects, and generalize them to achieve two additional important properties:
\begin{itemize}
    \item \textbf{Min-cost:} Our emulators generalize to the \emph{min-cost} multi-commodity flow problem, where each edge has an associated cost (independent of its capacity) and the multi-commodity flow must respect a certain cost budget. %This generalization to the min-cost setting is required to apply flow \emph{boosting} in the spirit of Garg-Konemann~\cite{garg2007faster}, whose $(1+\epsilon)$-approximate multi-commodity algorithm reduces to multiple shortest path computations. By combining our flow emulators with flow boosting, we can obtain constant-approximations to the value of the min-cost multi-commodity flow in $O((m+k)^{1+\epsilon})$ time for any $k$. 
    \item \textbf{Implicit Mappings:} Our flow emulators also support \emph{implicit} flow mappings from the emulator back to the original graph. In other words, we can even maintain an implicit solution to a constant-approximate multi-commodity flow, and \Cref{thm:informal-constapprox-cnc-flow} can be modified to output such an implicit representation for a flow of the approximated value. (Recall that implicit solutions are required to obtain any $o(mk)$ running time.) With this implicit solution, we can answer the following queries in $O((m+k)^{1+\epsilon})$ time: given any subset of the $k$ commodities, return the union of the flows of each of these commodities. As this is a single-commodity flow, it is representable explicitly within the allotted time.
\end{itemize}
The combination of the two generalizations will allow us to apply flow \emph{boosting} in the spirit of Garg-Konemann~\cite{garg2007faster} to obtain the above algorithms, and further allows us to obtain the above multi-commodity flow result subject to a cost constraint.

% In this paper, we show the existence of approximate (multi-commodity) flow emulators for undirected graphs, and obtain efficient algorithms to construct these objects. Our emulators have a \emph{low-step} guarantee: there exist approximate multi-commodity flows whose paths contain a small number of edges, bypassing the $O(mk)$ flow decomposition barrier. Our emulators also generalize to the \emph{min-cost} multi-commodity flow problem, where each edge has an associated cost (independent of its capacity) and the multi-commodity flow must respect a certain cost budget. This generalization to the min-cost setting is required to apply flow \emph{boosting} in the spirit of Garg-Konemann~\cite{garg2007faster}, whose $(1+\epsilon)$-approximate multi-commodity algorithm reduces to multiple shortest path computations. By combining our flow emulators with flow boosting, we can obtain constant-approximations to the value of the min-cost multi-commodity flow in $O((m+k)^{1+\epsilon})$ time for any $k$. %In particular, we bypass the $O(mk)$ flow decomposition barrier for estimating the value of a multi-commodity flow.

% Our flow emulators also supports \emph{implicit} flow mappings from the emulator back to the original graph. In other words, we can even maintain an implicit solution to a constant-approximate multi-commodity flow. (Recall that implicit solutions are required to obtain any $o(mk)$ running time.) With this implicit solution, we can answer the following queries in $O((m+k)^{1+\epsilon})$ time: given any subset of the $k$ commodities, return the union of the flows on each of these commodities, which is a single-commodity flow and hence representable explicitly within the allotted time.

\subsection{Our Techniques}
In the remainder of this section, we describe how we obtain our results in more detail. At a high-level, our approach is as follows. First, we compute low-step emulators by building on recent advances in length-constrained expander decompositions. Next, we use our low-step emulators to compute (implicit) flows on the original graph with potentially large congestion. Lastly, we use ``boosting'' to reduce this congestion down to a constant to get our final flow approximation.

\paragraph*{Step 1: Low-Step Emulators via Length-Constrained Expander Decompositions.}
Our techniques build on recent developments in \emph{length-constrained expander decompositions} ~\cite{haeupler2022hop,haeupler2022cut,Haeupler2023lenboundflow, haeupler2023parallel,haeupler2023length}. At a high level, $h$-length expanders are graphs with edge lengths and capacities for which any ``reasonable'' multi-commodity demand can be routed along (about) $h$-length paths with low congestion (by capacity). Informally, a reasonable demand is one where each demand pair $(s_i,t_i)$ is within $h$ by distance (so that sending flow from $s_i$ to $t_i$ along about-$h$-length paths is actually possible), and each vertex does not belong to too many demand pairs (so that the degree of the vertex is not an immediate bottleneck for congestion). Recent work~\cite{haeupler2022hop,haeupler2023length} has studied how to, in almost-linear time, compute \emph{length-constrained expander decompositions} which are length-increases---a.k.a.\ moving cuts---to the graph that make it an $h$-length expander. One caveat, however, is that these algorithms run in time polynomial in the \emph{length} parameter $h$ of the length-constrained expander decomposition. This is sufficient for unit-length graphs with small $h$, but for general graphs, edge lengths can be polynomially large, rendering such algorithms inefficient.

In this paper, we remove this polynomial dependency of $h$ by way of the above-mentioned low-step emulators. Specifically, we ``stack'' low-step emulators on top of each other with geometrically increasing lengths, similar to how hopsets are stacked in parallel algorithms~\cite{cohen2000polylog}. Each low-step emulator is responsible for flow paths of its corresponding length, and the union of all low-step emulators obeys all distance scales simultaneously.

Our construction of low-step emulators comes with an \emph{embedding} of the emulator into the base graph: each edge of the emulator maps to a small-length path in the base graph such that the set of all embedded paths has low congestion. When emulators are stacked on top of each other, an edge at the top level expands to a path at the previous level, each of whose edges expands to a path at the previous level, and so on. This hierarchical structure allows us to provide the aforementioned implicit representation of very long paths while keeping the total representation size small.

\paragraph*{Step 2: Flows on Emulators.}
Our next contribution is a fast algorithm that computes a multi-commodity flow on a low-step emulator, where an approximate flow with small representation size is indeed possible (since flow paths now have low step-length). We explicitly compute such a flow, and then (implicitly) map each flow path down the hierarchical structure to form our final implicit flow on the input graph. 

By setting parameters appropriately, we can guarantee a bicriteria approximation with constant-approximate cost and $n^\epsilon$-approximate congestion for any constant $\epsilon>0$. The $n^\epsilon$-approximate congestion appears in both the multi-commodity flow algorithm on a low-step emulator, and the hierarchical embeddings of the emulators into the base graph.

\paragraph*{Step 3: Boosting Away Congestion.}
Finally, through Garg and Konemann's approach~\cite{garg2007faster} based on multiplicative weight updates, we can \emph{boost} the congestion approximation of $n^\epsilon$ down to the cost approximation, which is constant. While Garg and Konemann's algorithm requires a near-linear number of calls to (approximate) shortest path, we only require roughly $n^\epsilon$ calls to constant-approximate cost, $n^\epsilon$-approximate congestion multi-commodity flow. Our final result is a multi-commodity flow with constant-approximate cost and congestion which is implicitly represented by the hierarchical emulator embeddings. Given any subset of commodities, we can then output the union of their flows by collecting the flow down the hierarchy of embeddings.

%%% old stuff
\iffalse
We introduce and show the existence of min-cost multi-commodity flow (MCMF) sparsifiers, i.e., for every graph $G$ with capacities and costs there exists a sparse graph $G'$ on the same vertex set such that any feasible multi-commodity flow in $G$ can be mapped to a flow routing the same demand with small congestion in $G'$ of approximately the same cost in $G'$ and vice versa. 

Our sparsifiers are step-reducing and guarantee that any approximately optimal flow in $G'$ can be routed over pathes with small number of steps/edges. 

For example, a sparsifier $G'$ with $m \cdot \poly(\log n)$ edges achieving a bicriteria $\poly(\log n)$ approximation in congestion and cost and guaranteeing that flows can be routed over flow-paths with $O(\log n)$ edges.

We also give essentially optimal tradeoffs bringing the cost approximation and step-length to and constant.% and extend the sparsifiers to vertex sparsifiers, i.e.,  given $k$ terminals there exists a MCMF vertex sparsifiers of size proportional to $k$ as well. 

We use these sparsifiers to give powerful new (min-cost) $k$-commodity flow algorithms which achieve a $O_{\eps}(1)$-approximation in $(m+k)^{1+\eps}$ time, shattering the $mk$ flow decomposition barrier.

Our sparsifiers also drastically improve the algorithmic theory of length-constrained expanders. In particular we give $m^{1+O(\eps)}$ time algorithms for length-constrained expanders, eliminating the polynomial dependency on $h$ of previous approaches. This makes $h$-length expanders a much more powerful tool for a host of MCF and MCMCF problems in capacitated graphs with costs.

%We introduce the notion of a min-cost flow sparsifiers $G'$ of a graph $G$, which approximately preserves the cost and flow-size of any multi-commodity in $G$.

%In addition to being sparse our sparsifiers are also step-reducing, i.e., any near-optimal min-cost flow can be routed via flow-paths with small number of edges. We also provide vertex sparsifiers for any terminal vertex set $T$ of close-to-linear size in $|T|$.

etc.
\fi
%%% end old stuff



==> arxivver/nodeweighting-demand-definitions.tex <==
\antti{the flow part got "a bit" more complicated because for cutmatches it seems to be necessary to handle concurrent and non-concurrent flows between node weightings, instead of just (s, t)-demands. In undirected graphs, it is not possible to just add a super-source and a super-sink, as other commodities could shortcut through these. Handling node weighting demands is not relevant for the end result of multi-commodity flow, but seems to be required to compute length-bounded expander decompositions without runtime dependence on $h$}

\antti{Writing these definitions in a very clear way is really challenging :(}

\antti{$k$-commodity node weighting demand = generalisation of a demand with support size $k$}

\antti{$(h, s)$-length sparsity here is a generalisation of $(h, s)$-length sparsity for $(s, t)$-demands. the "$t$-step" part just restricts the set of possible paths to consider. Really not sure about the notation there.}

\antti{Note: for algorithms with additive $k$ in the running time, we don't really know how to handle unbalanced node weighting demands (where $|A^{+}_i| \neq |A^{-}_i|$). Should we just define the problem away?}

\begin{definition}[Node Weighting Demand]\label{def:nodeweight-demand}
A $k$-commodity node weighting demand $\{(A^{+}_{i}, A^{-}_{i})\}_{i \in [k]}$ is a collection of $k$ node weighting pairs $(A^{+}_{i}, A^{-}_{i})$. The \textit{size} of the demand equals the sum of sizes of the smaller halves of the node weightings: $|\{(A^{+}_{i}, A^{-}_{i})\}_{i \in [k]}| = \sum_{i} \min(|A^{+}_{i}|, |A^{-}_{i}|)$. The node weighting demand is \textit{balanced} if $|A_{i}^{+}| = |A_{i}^{-}|$ for all $i$.
\end{definition}

\antti{Non-Concurrent flow for a node weighting demand is a "capped" flow from the supports of $A^{+}_i$'s to supports of $A^{-}_i$'s}

\begin{definition}[Node Weighting Non-Concurrent Multicommodity Flow]
A non-concurrent $k$-commodity flow $F = \sum_{i \in [k]} F_i$ on a node weighting demand $\{(A^{+}_{i}, A^{-}_{i})\}_{i \in [k]}$ is a multicommodity flow, such that for every commodity $i$,
\begin{itemize}
    \item For every vertex $v^{+}$, $\sum_{v^{-}} \mathrm{val}(F_{i, (v^{+}, v^{-})}) \leq A^{+}_{i}$, and
    \item For every vertex $v^{-}$, $\sum_{v^{+}} \mathrm{val}(F_{i, (v^{+}, v^{-})}) \leq A^{-}_{i}$.
\end{itemize}
\end{definition}

\antti{Concurrent flow has to send the same ratio of the maximum possible for every commodity. NOTE: It is NOT necessary for it to be a exact flow for some multiple of the node weighting demand. The "Concurrency" constraint only bounds the total flow values for every commodity.}

\begin{definition}[Node Weighting Concurrent Multicommodity Flow]
A concurrent $k$-commodity flow $F = \sum_{i \in [k]} F_i$ on a node weighting demand $\{(A^{+}_{i}, A^{-}_{i})\}_{i \in [k]}$ is a non-concurrent multicommodity flow for the node weighting demand, such that additionally, for some $\gamma$, for all $i \in [k]$,
\begin{equation*}
    \mathrm{val}(F_{i}) = \gamma \min(|A_{i}^{+}|, |A_{i}^{-}|).
\end{equation*}
\end{definition}

\begin{definition}[Sparsity of a Moving Cut of a Node Weighting Demand]\label{def:sparse-nodeweight-cut}
The $t$-step $(h, s)$-length sparsity of a moving cut $C$ with respect to a $k$-commodity node weighting demand is defined as
\begin{equation*}
\mathrm{spars}_{(t, h, s)}(C, \{(A^{+}_{i}, A^{-}_{i})\}_{i \in [k]}) = \max_{\text{valid } \{(A_{i, U}^{+}, A_{i, U}^{-})\}_{i \in [k]}} \frac{|C|}{|\{(A_{i, U}^{+}, A_{i, U}^{-})\}_{i \in [k]}|} 
\end{equation*}
where a "unmatched" node weighting demand $\{(A^{+}_{i, U}, A^{-}_{i, U})\}_{i \in [k]}$ is \textit{valid}, if for every $i \in [k]$,
\begin{itemize}
    \item The "unmatched" part is a subset of the original demand: $A_{i, U}^{+} \prec A_{i}^{+}$ and $A_{i, U}^{-} \prec A_{i}^{-}$,
    \item The "matched" part is equally large for both sides: $|A_{i}^{+} - A_{i, U}^{+}| = |A_{i}^{-} - A_{i, U}^{-}|$, and
    \item The cut $t$-step $hs$-separates any $t$-step $h$-close "unmatched" vertex pairs: for any $a_{+} \in \mathrm{supp}(A_{i, U}^{+})$ and $a_{-} \in \mathrm{supp}(A_{i, U}^{-})$ such that $\mathrm{dist}_{G, t}(a_{+}, a_{-}) \leq h$, $\mathrm{dist}_{G - C, t}(a_{+}, a_{-}) \geq hs$.
\end{itemize}
\end{definition}

\begin{definition}[single-commodity length-constrained cutmatch]\label{def:cutmatch-new}
A $(t, \hat{s})$-step $(h, s)$-length $\phi$-sparse cutmatch with congestion slack $\kappa$ for a node weighting pair $(A^+, A^-)$ consists of:
\begin{itemize}
    \item A $t$-step $(h, s)$-length $\phi$-sparse moving cut $C$ of $\{(A^{+}, A^{-})\}$, and
    \item A $t \hat{s}$-step $hs$-length congestion-$\frac{\kappa}{\phi}$ flow $F$ from $A^{+}$ to $A^{-}$, such that for any pair $(a_{+}, a_{-})$ of vertices that are $t$-step $h$-close in $G$, either
    \begin{itemize}
        \item One vertex is \textit{saturated}: $A^{+}(a^{+}) = \sum_{v} \mathrm{val}(F_{(a^{+}, w)})$ or $A^{-}(a^{-}) = \sum_{v} \mathrm{val}(F_{(v, a^{-})})$, or
        \item The vertices are $t$-step $hs$-separated by $C$: $\mathrm{dist}_{G - C, t}(a^{+}, a^{-}) \geq hs$.
    \end{itemize}
\end{itemize}
\end{definition}

% ANTTI: names for the node weightings? (A, A'), (A^+, A^-), (A, B) ??
\begin{definition}[multi-commodity length-constrained cutmatch]\label{def:mc-cutmatch-new}
A $(t, \hat{s})$-step $(h, s)$-length $\phi$-sparse $k$-commodity cutmatch with congestion slack $\kappa$ for node weighting demand $\{(A^{+}_{i}, A^{-}_{i})\}_{i \in [k]}$ consists of:
\begin{itemize}
    \item A $t$-step $(h, s)$-length $\phi$-sparse moving cut $C$ of $\{(A^{+}, A^{-})\}$, and
    \item A $t \hat{s}$-step $hs$-length congestion-$\frac{\kappa}{\phi}$ multicommodity flow $F = \sum_{i \in [k]} F_i$ where $F_i$ is from $A^{+}_i$ to $A^{-}_i$, such that for every commodity $i \in [k]$ and any pair $(a_{+}, a_{-})$ of vertices that are $t$-step $h$-close in $G$, either
    \begin{itemize}
        \item One vertex is \textit{saturated}: $A_i^{+}(a^{+}) = \sum_{v} \mathrm{val}(F_{i, (a^{+}, w)})$ or $A_i^{-}(a^{-}) = \sum_{v} \mathrm{val}(F_{i, (v, a^{-})})$, or
        \item The vertices are $t$-step $hs$-separated by $C$: $\mathrm{dist}_{G - C, t}(a^{+}, a^{-}) \geq hs$.
    \end{itemize}
\end{itemize}
\end{definition}

\subsection{Step-Bounded High-Commodity Cutmatch}

This subsection presents a cutmatch algorithm with \textbf{additive}, not multiplicative dependency on the number of commodities $k$., for \textbf{balanced} node weighting demands: demands where $|A_{i}^{+}| = |A_{i}^{-}|$.

\antti{To get rid of the restriction to balanced demands, replace expander decompositions with sparse cuts? How to do this is not clear.}

The cutmatch algorithm takes as input pairs of node weightings $\{(A_i^+, A_i^-)\}_{i \in [k]}$, one for each commodity. As a subroutine, it needs to perform length-bounded expander routing, which uses demands as input. \Cref{alg:nodeweight-demand-conversion} is a simple algorithm that converts the node weighting pairs to a maximal demand: no $h$-close pairs with nonzero node weighting can remain after subtracting the demand.

\begin{lemma}\label{lem:nodeweight-demand-conversion-correctness}
Given a graph $G$ with edge lengths $l$ and capacities $u$, a node weighting demand $\{(A^{+}_i, A^{-}_i)\}_{i \in [k]}$, a length bound $h$ and a tradeoff parameter $\epsilon \in (0, 1)$, \Cref{alg:nodeweight-demand-conversion} returns length-$O(h / \eps)$ demands $D_i$
\begin{itemize}
    \item from $A_i^+$ to $A_i^-$: $\mathrm{load}_{+}(D_i) \prec A_i^+$ and $\mathrm{load}_{-}(D_i) \prec A_i^-$,
    \item of support size $\mathrm{supp}(D_i) \leq \mathrm{supp}(A_i^+) + \mathrm{supp}(A_i^-)$,
\end{itemize}
such that the unmatched parts are $h$-separated:
\begin{equation*}
    \mathrm{dist}_{G}(\mathrm{supp}(A_{i}^{+} - \mathrm{load}_{+}(D_i)), \mathrm{supp}(A_{i}^{-} - \mathrm{load}_{-}(D_i))) > h.
\end{equation*}
The algorithm does $\tilde{O}(N^{\eps} \cdot (m + \sum_i \mathrm{supp}(A_i^+ + A_i^-)))$ work and has depth $\tilde{O}(N^{\eps})$. The returned demands are integral if the input node weightings are integral.
\end{lemma}

\begin{algorithm}\label{alg:nodeweight-demand-conversion}
\caption{Node Weighting Pair $\rightarrow$ Demand Conversion}
\textbf{Input: } Graph $G$, node weighting demand $\{(A^{+}_i, A^{-}_i)\}_{i \in [k]}$, length bound $h$, tradeoff parameter $\epsilon \in (0, 1)$.\\
\textbf{Output: } Length-$O(h / \eps)$ integral demands $D_i$ from $A^+_i$ to $A^-_i$ of support size $\mathrm{supp}(D_i) \leq \mathrm{supp}(A^+_i) + \mathrm{supp}(A^-_i)$, such that the unmatched parts of each node weighting are $h$-separated.

\begin{enumerate}
    \item Let $\mathcal{N}$ be a neighbourhood cover of covering radius $h$, diameter $h \cdot O(1 / \eps)$ and width $\tilde{O}(N^{\eps})$, computed using \antti{theorem}.
    \item For $i \in [k]$, in parallel, let $D_i \leftarrow 0$.
    \item For every clustering $\mathcal{S} \in \mathcal{N}$:
    \begin{enumerate}
        \item For every commodity $i \in [k]$, in parallel,
        \begin{enumerate}
            \item For every cluster $S \in \mathcal{S}$ with nonzero intersection with $\mathrm{supp}(A^{+}_i + A^{-}_i)$, in parallel,
            \begin{enumerate}
                \item Let $D'$ be a greedy maximal matching from $A^{+}_i |_S$ to $A^{-}_i |_S$.
                \item Let $D_i \leftarrow D_i + D'$.
                \item Let $A^{+}_i \leftarrow A^{+}_i - \mathrm{load}_{+}(D_i)$.
                \item Let $A^{-}_i \leftarrow A^{-}_i - \mathrm{load}_{-}(D_i)$.
            \end{enumerate}
        \end{enumerate}
    \end{enumerate}
    \item Return $\{D_i\}_{i \in [k]}$.
\end{enumerate}
\end{algorithm}

\begin{proof}
    Every produced demand is from $A^+_i$ to $A^-_i$, and the demand's load is subtracted from the node weightings, thus the final demand $D_i$ respects the node weightings.

    A greedy maximal matching is produced by repeatedly taking two vertices $u, v \in S$ with $A^+_i(u) > 0$ and $A^-_i(v) > 0$, and adding demand between them equal to $\min(A^+_i(u), A^-_i(v))$. Thus, every vertex pair with nonzero demand reduces the support size of either $A^+_i$ or $A^-_i$ by one, and $\mathrm{supp}(D_i) \leq \mathrm{supp}(A_i^+) + \mathrm{supp}(A_i^-)$. This guarantees the output demand is integral if the node weightings are.
    
    The demand has length $O(h / \eps)$, as any cluster in $\mathcal{N}$ has at most this diameter, and any demand is only ever nonzero for pairs of vertices that appear together in a cluster.
    
    As the demand $D'$ produced is a greedy maximal matching, after handling a cluster, commodity pair $(S, i)$, either $A^{+}_i(S) = 0$ or $A^{-}_i(S) = 0$. Since the neighbourhood cover has covering radius $h$, any two vertices at distance at most $h$ from each other appear together in some cluster. Thus, the distance from the unmatched part of $A^+_i$ to the unmatched part of $A^-_i$ is greater than $h$.

    Producing a greedy maximal matching can be done with $\tilde{O}(|\mathrm{supp}(A_i^+) \cap S| + |\mathrm{supp}(A_i^-) \cap S|)$ work and $\tilde{O}(1)$ depth, thus as the neighbourhood cover has width $N^{\epsilon}$, the work and depth outside of computing the neighbourhood cover equal $\tilde{O}(N^{\eps} \cdot \sum_i \mathrm{supp}(A_i^+ + A_i^-))$ and $\tilde{O}(N^{\eps})$. \antti{Theorem} gives an algorithm for constructing the neighbourhood cover with the desired parameters, with work $\tilde{O}(m \cdot N^{\eps})$ and depth $\tilde{O}(N^{\eps})$.
\end{proof}

\begin{lemma}\label{lem:highcomcutmatch}
Given a graph $G$ with edge lengths $l$ and capacities $u$, an \textbf{integral balanced} node weighting demand $\{A^{+}_i, A^{-}_i\}_{i \in [k]}$, a length bound $h$, a sparsity parameter $\phi$ and tradeoff parameters $\epsilon, \epsilon' \in (0, 1)$, \Cref{alg:highcomcutmatch} returns a $(h, s)$-length $\phi$-sparse multicommodity cutmatch with length slack $s = (1 / \eps)^{O(1 / \eps')}$, congestion slack $\kappa = (\frac{N^{\poly(\eps)}}{\poly(\eps)})^{O(1 / \eps')}$ and flow support size
\begin{equation*}
    \tilde{O}((m + \sum_i \mathrm{supp}(A_i^{+}) + \mathrm{supp}(A_i^{-})) \cdot N^{\poly(\epsilon, \epsilon')}).
\end{equation*}
The algorithm does $\dots$ work and has depth $\dots$.
\end{lemma}

\begin{algorithm}\label{alg:highcomcutmatch}
\caption{High-Commodity Cutmatch}
\textbf{Input: } Graph $G$ with edge lengths $l$ and capacities $u$, integral balanced node weighting demand $\{(A^{+}_i, A^{-}_i)\}_{i \in [k]}$, length bound $h$, sparsity parameter $\phi$, tradeoff parameters $\epsilon, \epsilon' \in (0, 1)$.\\
\textbf{Output: } A $(h, s)$-length $\phi$-sparse multi-commodity cutmatch with length slack $s = (1 / \eps)^{O(1 / \eps')}$, congestion slack $\kappa = \left(\frac{N^{\poly(\eps)}}{\poly(\eps)}\right)^{O(1 / \eps')}$ and flow support size $\tilde{O}((m + \sum_i \mathrm{supp}(A_i^{+}) + \mathrm{supp}(A_i^{-})) \cdot N^{\poly(\epsilon, \epsilon')})$.

\begin{enumerate}
\item For $i \in [k]$, in parallel:
\begin{itemize}
    \item Let $F_i \leftarrow 0$.
    \item Let $A^{+}_{i, U} \leftarrow A^{+}_i$ and $A^{-}_{i, U} \leftarrow A^{-}_i$.
    \item Let $A^{+}_{i, M} \leftarrow 0$ and $A^{-}_{i, M} \leftarrow 0$.
\end{itemize}
\item Let $s' := (1 / \eps)^{O(1 / \eps')}$ and $\kappa' := \left(\frac{N^{\poly(\eps)}}{\poly(\eps)}\right)^{O(1 / \eps')}$, with appropriate asymptotics.
\item Let $\phi' := \phi \cdot \frac{1}{4 \kappa'} \cdot \frac{s' - 1}{s - 1}$.
\item Repeat:
\begin{enumerate}
\item Let $C$ be a $(hs'^2, s')$-length $(\phi', \kappa')$-expander decomposition for $\sum_i (A_{i, U}^+ + A_{i, U}^-)$, computed using \antti{expander decomposition algorithm}.
\item Let $\{D_i\}_{i \in [k]}$ be length-$hs'^2$ demands from \Cref{alg:nodeweight-demand-conversion} on the graph $G - C$, length bound $hs'$, tradeoff parameter $\epsilon$ and node weighting pairs $\{(A_{i, U}^{+}, A_{i, U}^{-})\}_{i \in [k]}$.
\item Let $F'$ be a multi-commodity flow for $D = \sum D_i$ in $G - C$ with length $O(hs'^4)$ and congestion $\tilde{O}\left(\phi'^{-1} \cdot \kappa' \right)$, computed using \antti{routing in a router algorithm}. % \Cref{thm:routingexpander}.
\item For $(a, b) \in \mathrm{supp}(D)$, in parallel:
\begin{enumerate}
    \item Greedily split $F'(a, b)$ into $\sum_i F'_i(a, b) = F'(a, b)$ such that $\mathrm{vol}(F'(a, b)) = D_i(a, b)$.
    \item For $i$ with $D_i(a, b) > 0$, in parallel:
    \begin{itemize}
        \item Let $F_i(a, b) \leftarrow F_i(a, b) + F'_i(a, b)$.
        \item Subtract $D_i(a, b)$ from $A_{i, U}^{+}(a)$ and add it to $A_{i, M}^{+}(a)$.
        \item Subtract $D_i(a, b)$ from $A_{i, U}^{-}(b)$ and add it to $A_{i, M}^{-}(b)$.
    \end{itemize}
\end{enumerate}
\item If $|C| \cdot \frac{s - 1}{s' - 1} \leq \frac{\phi}{2} \cdot \sum_i |A_{i, U}^+ + A_{i, U}^-|$:
\begin{itemize}
    \item return $C \cdot \frac{s - 1}{s' - 1}$ and $F = \sum_i F_i$.
\end{itemize}
\end{enumerate}
\end{enumerate}
\end{algorithm}

\begin{proof}
    We will show that the loop (4) is iterated at most $O(\log N)$ times before the algorithm returns a valid $(h, s)$-length cutmatch. First, we quickly argue that proving this is sufficient:
    \begin{itemize}
        \item \textbf{Size of cut.} As the node weighting demand is balanced, $\min(|A_{i, U}^{+}|, |A_{i, U}^{-}|) = \frac{1}{2} |A_{i, U}^{+} + A_{i, U}^{-}|$, and the algorithm only returns if the cut has the desired size.
        \item \textbf{Separation of unmatched node weight.} The demands $D_i$ produced by \Cref{alg:nodeweight-demand-conversion} guarantee that $\mathrm{supp}(A_{i, U}^+ - \mathrm{load}_{+}(D_i))$ is $hs'$-far in $G - C$ from $\mathrm{supp}(A_{i, U}^- - \mathrm{load}_{-}(D_i))$. The returned cut is multiplied by $\frac{s - 1}{s' - 1}$, thus with the returned cut, the unmatched parts are $hs$-separated.
        \item \textbf{Flow length and congestion.} The demands prodyced by \Cref{alg:nodeweight-demand-conversion} are length $hs'^2$ in $G - C$, which is a length-$hs'^2$ $\phi'$-expander. Thus, \Cref{thm:routingexpander} produces flows satisfying the demand of length $O(hs' \cdot s'^3) = hs$ and congestion $\tilde{O}(\phi'^{-1} \cdot \kappa')$. We let $\kappa = O(\kappa'^2 s' \log N)$. Then, as the returned flow is a sum of at most $O(\log N)$ flows of length $hs$ and congestion $\kappa / O(\log N)$, it has the desired length and congestion.
        \item \textbf{Flow support size.} The individual flows $F'$ produced by \Cref{thm:routingexpander} have support size $\tilde{O}((m + \mathrm{supp}(D)) \cdot N^{\poly(\epsilon, \epsilon')})$. Splitting the flow for $D = \sum D_i$ at (ii) into individual flows increases the support size by at most the number of commodities with nonzero $D_i(a, b)$, and \Cref{alg:nodeweight-demand-conversion} guarantees $\mathrm{supp}(D_i) \leq \mathrm{supp}(A_i^+) + \mathrm{supp}(A_i^-)$. Thus, the resulting in support size is $\tilde{O}((m + \sum_i \mathrm{supp}(A_i^{+}) + \mathrm{supp}(A_i^{-})) \cdot N^{\poly(\epsilon, \epsilon')})$, as desired. The $O(\log N)$ from summing up multiple flows is absorbed into the $\tilde{O}(1)$-factor.
        \item \textbf{Work and depth.} \antti{todo}.
    \end{itemize}

    \antti{this is incredibly annoying. The "length" of the cuts changes, but there is no way in the notation of denoting based on what length the cut's size is computed.}
    
    It remains to show the number of iterations of loop (4) is $O(\log N)$. The \antti{expander decomposition algorithm} guarantees that
    \begin{equation*}
        |C| \leq \kappa' \phi' \cdot \sum_i |A_{i, U}^+ + A_{i, U}^{-}| = \frac{1}{2} \cdot \frac{\phi}{2} \cdot \frac{s' - 1}{s - 1} \cdot \sum_i |A_{i, U}^+ + A_{i, U}^{-}|.
    \end{equation*}
    Thus, as long as $\sum_i |A_{i, U}^+ + A_{i, U}^-|$ drops by at most a multiplicative factor of $2$, $|C|$ has the desired size, and the algorithm returns. On the other hand, as all node weightings start and always remain integral, this must happen after $O(\log \sum_i |A_{i}^+ + A_{i}^-|) = O(\log N)$ iterations.
\end{proof}

==> arxivver/notation-and-naming-conventions.tex <==
\section{Naming / Notation Questions}

Suggestions:
\begin{itemize}
    \item Sparsifier vs. emulator: I now tend towards emulator mainly because sparseness is very much not the most important property (but step-reducing), sparsifiers tend to be (reweighted) sub-graphs - which is not possible for us

    Only counter point: sparsifiers are more common and people know what vertex sparsifiers are...

    \item terminal vs vertex emulator/sparsifier: 

    I would advocate for terminal. 

    given that we mostly talk about nodes saying vertex sparsifier is weird, terminal is equally(?) self-explanatory.

    \item For consistency with past the proposal was:

    steps = number of edges
    length = sum of length/weights

    use hop as equivalent for length (not step) largely restricted (as much as possible) to settings with unit length edges

    
    \item Proposal: 
    
    Generally talk about about length-constrained expanders, emulators, routings, etc.? For example 
    LC-expander, $(h,s)$-LC expander, $h-LC$ $t$-step emulator, ...

    Go away from $h$-hop, hop-bounded (constrained is more accurate),...

    \item Use deg for the capacitated degree

    for the very rare case where we want to talk about number of adjacent edges, what shall we use (neighborhood function $|\Gamma(v)|$?)

    \item Proposal: 

    Operate on node-weightings only with deg being the default node-weighting

    however, I'm not sure we want to completely eliminate the use of self-loops? It makes talking about routings more concrete... (maybe localize this as much as possible)

    


    \item Proposal:

    Go away from length profiles? 
    Flow-mappings are more precise and concrete and we want to talk about their properties efficiencies a bunch. 

    If useful as a proof tool, keep both?

    \item Step-Reducing vs. Step-Constrained vs. Step-Bounded vs. $t$-step / low-step

\end{itemize}


==> arxivver/offline_dyn.tex <==

\section{Offline $O(1)$-Approx Fully Dynamic Min Cost Flow}



In the offline fully-dynamic min-cost flow problem, we are given an initial empty graph $G_{0}$ with $n$ vertices and a sequence $U$ of $m$ operations consisting of edge insertions, edge deletions, and queries between two vertices. Let $U_{\le i}$ denote the first $i$ operations of $U$ and $G_{i}$ denote the graph after performing edge updates in $U_{\le i}$. Our task is output, for each query $(s,t)$ in the sequence $U$, output a $(\alpha_{\mathrm{cost}},\alpha_{\mathrm{value}})$-approximate value of the min-cost $(s,t)$-flow in the current graph (i.e. in $G_{i}$ if the query is the $i$-th operation in the $U$).
\begin{thm}
There exists an algorithm for the offline fully-dynamic min cost flow that can return $(O(1),n^{\eps})$-approximate answers all queries in $O(mn^{\eps})$ total time.
\end{thm}



\begin{itemize}
\item Point: Application of vertex sparsifiers 
\item Outline:
\begin{itemize}
\item Define Min-cost flow emulator. 
\item Low-Step emulator is a min-cost flow emulator. 
\item Prove that min-cost flow emulator is composable.
\begin{itemize}
\item (Def 2.4 of https://www.dropbox.com/s/kcx0a1hvsbxii6s/Local\_Sparsifiers.pdf?dl=0)
\end{itemize}
\item Apply blackbox get offline-dynamic min cost flow.
\end{itemize}
\end{itemize}

